Incremental Property Directed Reachability

Property Directed Reachability (PDR) is a widely used technique for formal verification of hardware and software systems. This paper presents an incremental version of PDR (IPDR), which enables the automatic verification of system instances of incremental complexity. The proposed algorithm leverages the concept of incremental SAT solvers to reuse verification results from previously verified system instances, thereby accelerating the verification process. The new algorithm supports both incremental constraining and relaxing; i.e., starting from an over-constrained instance that is gradually relaxed. To validate the effectiveness of the proposed algorithm, we implemented IPDR and experimentally evaluate it on two different problem domains. First, we consider a circuit pebbling problem, where the number of pebbles is both constrained and relaxed. Second, we explore parallel program instances, progressively increasing the allowed number of interleavings. The experimental results demonstrate significant performance improvements compared to Z3's PDR implementation SPACER. Experiments also show that the incremental approach succeeds in reusing a substantial amount of clauses between instances, for both the constraining and relaxing algorithm.

==> 06_encoding.tex <==
%!TEX root = main.tex

\section{Incremental Property Directed Reachability}
\label{sec:ipdr}



==> sections/experiments/compare.tex <==
\subsection{Comparison}
Compared against \cite{quantum-pebbling}.

\begin{itemize}
    \item Given a DAG and $k$ pebbles. Find a valid pebbling, with a minimum number of steps.
    \item Given a DAG an $k$ pebbles. Does a valid strategy with $k$ steps exist.\begin{itemize}
        \item Starts at $k$ pebbles and $steps \gets k$
        \item If this fails or solver reaches 120 second timeout, $steps \gets steps + 1$ and retry
    \end{itemize}
    
    \subsubsection{Table Results (Show-case B)}
    Contains runs with H gate from Algorithm 4 in \cite{genus-operators}, and ISCAS85 benchmarks.
    
    Show-case $A$ in \cite{pebbling} mentions that they assume modular addition, subtraction, multiplication and squaring have a quantum implementation. Cost is given in terms of gates and ancillae. Show-case $B$ does not explicitly mention this.
    
    \paragraph{Multi-bit Hadamard Gates} 
    Modulare addition/subtraction implemented in a \textit{mockturtle}\footnote{https://github.com/lsils/mockturtle} XOR-majority graph. XMG has an efficient mapping into quantum circuits. Produces XMG graph, exported in DOT. Read into nodes/edges.
\end{itemize}


==> sections/experiments/copy.tex <==
\subsection{Constrained Copying in Relaxing IPDR} \label{exp:copy}
\input{sections/experiments/results/relax/simple.tex}


==> sections/experiments/pebbling.tex <==
\subsection{Reversible Pebbling Game} \label{exp:pebbling}
	The Reversible Pebbling Game that was introduced in
	\autoref{imp:pebbling} is used to perform both the constraining and relaxing
	versions of \ipdr from \autoref{ipdr}.

	\ipdr will be compared against three other algorithms. The constraining and
	relaxing versions will be denoted as \cipdr and \ripdr respectively. The
	underlying \pdr implementation that \ipdr used was written mainly according
	to the specifications in \autoref{bg:pdr} and \autoref{exp:imp}, mainly
	inspired by the work of Bradley \cite{ic3bradley} and Niklas Een et al.
	\cite{efficient-pdr}. It was then adjusted to allow for the features
	described in \autoref{ipdr}.
	
	\paragraph{Internal}
	The first is a series of multiple executions of the same underlying \pdr
	implementation and settings that \ipdr uses, only without any of the
	optimizations from \autoref{ipdr}. This comparison should give the cleanest
	insights into the effects of the \ipdr optimizations.
	
	\paragraph{Spacer} 
	The second is a comparison against Z3's \spacer engine \cite{spacer, z3}.
	\spacer  uses an \smt-solver to find fixedpoints or traces for a given
	property. The main structure of the Boolean encoding can be
	reused in the Constrained Horned Clauses that encode the system
	for the \spacer engine in
	\autoref{encoding:horn:pebbling:formula}. The main difference
	is the usage of the \ttfunction{state} Boolean function, which
	returns \textit{true} if an assignment of variables form a state in
	the system. The initial state is simply declared to be a state
	of the system, any transition from a state in the system is
	declared under a cardinality constraint, and the final state is
	defined by declaring that any state under $\neg \form P$ leads
	to $\bot$.

	 Since \spacer does not expose its internal state in any obvious or safe
	 manner, this version does not implement any of the \ipdr optimizations.
	 Thus, it serves as a reference for the efficiency of the custom \pdr
	 implementation that is employed by \ipdr.

	\paragraph{Bounded Model Checking}
	Last, is a \bmc algorithm, written according to specifications given by
	Giulia Meuli et al. \cite{quantum-pebbling}. This employs the same Z3
	\sat-solver to perform bounded model checking. Notably, this implementation
	uses a 120 second timeout on each step of \bmc, concluding that no trace
	exists if it is ever reached. This means that this approach cannot prove a
	true optimum for the number of pebbles used, as is typical for a \bmc
	approach.

\subsubsection{Benchmarks}
	The \DAG used for the Reversible Pebbling Problem in this thesis were
	obtained by generating a dependency graph for each computation in a
	quantum circuit. Whenever there is a gate with inputs $i_0, i_1, \ldots$
	
	The circuits themselves were taken from the
	Reversible Logic Synthesis Benchmarks Page \cite{rls-benchmarks}.
	This page lists several ``Families" of circuits of increasing size
	and complexity. The specific circuits used in the experimental
	evaluation of this thesis were chosen based on which could be
	completed in a reasonable time in a round of preliminary testing on
	available hardware. The following circuits were used:
	
	\begin{itemize}
		\item ham3tc.tfc
		\item mod5d1.tfc
		\item 4b15g\_1.tfc
		\item gf2\textasciicircum3mult\_11\_47.tfc
		\item gf2\textasciicircum4mult\_19\_83.tfc
		\item 5mod5tc.tfc
		\item gf2\textasciicircum5mult\_29\_129.tfc
		\item 5bitadder.tfc
		\item ham7tc.tfc
		\item gf2\textasciicircum10mult\_109\_509.tfc
	\end{itemize}
	
	%        \begin{itemize}
		%            \item 4b15g\_1.tfc
		%            \item 5bitadder.tfc
		%            \item 5mod5tc.tfc
		%            \item gf2\textasciicircum10mult\_109\_509.tfc
		%            \item gf2\textasciicircum3mult\_11\_47.tfc
		%            \item gf2\textasciicircum4mult\_19\_83.tfc
		%            \item gf2\textasciicircum5mult\_29\_129.tfc
		%            \item gf2\textasciicircum6mult\_41\_185.tfc
		%            \item gf2\textasciicircum7mult\_55\_251.tfc
		%            \item gf2\textasciicircum8mult\_85\_341.tfc
		%            \item gf2\textasciicircum9mult\_89\_413.tfc
		%            \item ham15tc1.tfc
		%            \item ham3tc.tfc
		%            \item ham7tc.tfc
		%            \item mod\_4mod5-n5-gc4-qc13.tfc
		%            \item mod5d1.tfc
		%            \item mod\_5mod5-n6-gc7-qc429.tfc
		%            \item rd32.tfc
		%        \end{itemize}

	
\subsubsection{Display}
	\autoref{fig:pebbling:constrain:all} and \autoref{fig:pebbling:relax:all}
	show the overall runtimes of the tested algorithms. More detailed figures can
	be found in \autoref{app:exp:stats}, which are also discussed here. 

	A table shows the
	runtimes for each benchmark, rounded to three decimal points. The last
	column, ``Improvement" shows the percentage reduction in runtime from the
	naive \ipdr version, compared to the \ipdr version with the optimizations
	from \autoref{ipdr}.
	
\subsubsection{Constraining IPDR Results}
	\input{sections/experiments/results/constrain/all.tex}
	\autoref{fig:pebbling:constrain:all} contains the overall results for the
	constraing version of \ipdr. Over half of the tested benchmarks achieve a
	speedup using the constraining \ipdr algorithm, ranging from roughly $30\%$
	to $60\%$ of the naive \cipdr runtime. This is also a speedup which falls
	outside of the standard deviation of naive \ipdr.
	
	The least effect was observed with the smallest benchmark \texttt{ham3tc},
	which shows a negligible difference that does not show on the rounded, three
	decimal representation.
	
	\cipdr actually shows a degradation of performance in the
	\texttt{gf2\^{}3mult\_11\_47}, \texttt{gf2\^{}4mult\_19\_83} and
	\texttt{gf2\^{}5mult\_29\_129} benchmarks. It is noteworthy that these are
	derived from circuits that compute the same Galois Field Multiplication
	function for a variable input size.
	
	The \spacer engine starts out in line with the smaller benchmarks, but
	quickly outperforms the naive \cipdr implementation. In some of the larger
	case, where \spacer outperforms naive \cipdr, the \cipdr algorithm
	compensates and achieves similar runtimes to \spacer. Namely in the
	\texttt{4b15g\_1} and \texttt{ham7tc}.

	\paragraph{Constraining ham7tc}
	\input{sections/experiments/results/constrain/ham7tc}
	Figures \ref{fig:pebbling:constrain:ham7:cti} and
	\ref{fig:pebbling:constrain:ham7:oblsat}.
	show some more detailed statistics from the \texttt{ham7tc} experiment, which was the most promising for the constraining version of \ipdr.
	
	\autoref{fig:pebbling:relax:ham7:cti} shows that \cipdr decreases the number of counterexamples \pdr considers across all iterations after the first, with a corresponding decrease in runtime. The graph shows that the \cipdr and naive versions have a similar exponential scaling in runtimes as the iterations progress. \autoref{fig:pebbling:constrain:ham7:oblsat} shows a similar relation for the number of handled obligations and \sat-queries.
	
	The runtimes of the different experimental samples were more consistent for \cipdr than it was for the naive implementaiton, as the standard deviations reported in the table of \autoref{fig:pebbling:relax:ham7:cti} are considerably lower.
	
	\paragraph{Constraining gf2\^{}5mult\_29\_129}
	\todo{examine good and bad case (ham7tc and gf2)}
	
\subsubsection{Relaxing IPDR Results}
	\input{sections/experiments/results/relax/all.tex}

	\autoref{fig:pebbling:relax:all} shows no significant improvement in most
	benchmarks. In fact, some benchmarks show a notable degradation in runtime,
	namely for \texttt{gf2\^{}5mult\_29\_129} and \texttt{ham7tc}. The only positive result is for the \texttt{5bitadder} experiment.
	
	Compared to the constraining algorithm, the relaxing algorithm tends to perform much fewer iterations. It seems that the minimum number of pebbles that can be used for a valid strategy lies much closer to the starting point of the relaxing algorithm than it does to that of the constraining algorithm. \todo{table/figure}
	Furthermore, most relaxing iterations seem trivial to solve until the algorithm gets close to the first trace.

	\paragraph{Relaxing 5bitadder}
	\input{sections/experiments/results/relax/5bitadder-results.tex}
	Figures \ref{fig:pebbling:relax:5bit:cti},
	\ref{fig:pebbling:relax:5bit:oblsat} and \ref{fig:pebbling:relax:5bit:copy}
	show some more detailed statistics from the \texttt{5bitadder} experiment,
	which was the only one to significantly decrease the runtime.

	\autoref{fig:pebbling:relax:5bit:cti} shows that the \cipdr version needs to
	consistently considers fewer counterexamples than the naive version, but there is only a significant decrease of the runtime in the last iteration.
	
	\autoref{fig:pebbling:relax:5bit:obl} reveals that these decreases do not correspond to notable decrease in the number of obligations that need to be considered until the final iteration. While this decrease does result in fewer \sat-queries and time spent in the \sat-solver, this speedup is not quite of the same order as the decrease in obligations.

	\autoref{fig:pebbling:relax:5bit:copy} shows that clauses learned in one
	iteration can be consistently carried over to the next. Cubes can not be blocked as far as they were before, as they are now more front-loaded in the candidate sequence, but around half of the information remains valid.
	
	\paragraph{Relaxing ham7tc}
	Figures \ref{fig:pebbling:relax:ham7:cti},
	\ref{fig:pebbling:relax:ham7:oblsat} and \ref{fig:pebbling:relax:ham7:copy}
	show the detailed statistics for the \texttt{ham7tc} input, which produced
	one the more promising in constraining \ipdr but performed the worst under
	relaxing \ipdr.

	\input{sections/experiments/results/relax/ham7tc.tex}

	\paragraph{Relaxing 5mod5tc}
	Figures \ref{fig:pebbling:relax:5mod5tc:cti},
	\ref{fig:pebbling:relax:5mod5tc:oblsat} and
	\ref{fig:pebbling:relax:5mod5tc:copy} show the detailed statistics for the
	\texttt{5mod5tc} input, which did not produce any significant change in
	runtime with relaxing \ipdr.

	The amount of counterexamples in \autoref{fig:pebbling:relax:5mod5tc:cti} and
	obligations handled by \pdr in \autoref{fig:pebbling:relax:5mod5tc:obl} are
	still consistently decreased using \ripdr. Most of the work is done for
	pebbling constraints 5 and 6, where this decrease can be most clearly
	observed. However, it can be seen that the iteration constraint 6 does have s
	shorter runtime despite this decrease.

	Looking at \autoref{fig:pebbling:relax:5mod5tc:sat}, it can be seen this
	decrease does not result in corresponding in the number of \sat-solver
	calls made. For constraint 5, the number of \sat-solver calls is slightly
	lower, which corresponds to a similar decrease in runtime. For constraint 6,
	the reverse is true. \todo{MIC attempts is slightly lower in naive for 5 and 6}

		\input{sections/experiments/results/relax/5mod5tc.tex}

\subsubsection{Binary Search Results}
	\input{sections/experiments/results/binary/all.tex}


==> sections/experiments/peter.tex <==
\subsection{Peterson Protocol Results}
\autoref{fig:peter:relax:all} shows the overall runtimes for three instances of
the Peterson Protocol from \autoref{imp:peterson}: \ttfunction{Peterson}[2],
\ttfunction{Peterson}[3] and \ttfunction{Peterson}[4]. The runtimes increase
exponentially for higher number of processes, making \ttfunction{Peterson}[4]
the greatest instance that was feasible to run.

The runtime also limited the bound on the number of context switches that was
feasible to run: \ttfunction{Peterson}[2] was verified up to a bound of 10
switches, \ttfunction{Peterson}[3] to a bound of 4 and \ttfunction{Peterson}[4]
to 3.

\verb|this is relax with copy constrain.|

\ttfunction{Peterson}[2] improved the most under \ripdr, improving its runtime
by almost 60\%. \ttfunction{Peterson}[3] and \ttfunction{Peterson}[4] both
showed a similar improvement of around 30\%.


\input{sections/experiments/results/peter/all.tex}

\subsubsection{4 processess}
	\input{sections/experiments/results/peter/4proc}


==> sections/experiments/results/constrain/gf2_129.tex <==
\begin{figure}[ht]
    \centering
    \begin{tabular}
        {|r|rr|r|}
        \hline
        & \cipdr & Naive \cipdr & Improvement \\\hline
		avg time & 1243.961 s & 760.006 s & -63.68 \% \\
		std dev time & 148.944 s & 351.693 s &  \\
		avg incremental time & 4.834 s &  &  \\
		std dev incremental time & 0.552 s &  &  \\
		max inv constraint & 7 & 7 &  \\
		min inv level & 19 & 7 & 0.00 \% \\
		min strat marked & 8 & 8 &  \\
		min strat length & 47 & 49 & 4.08 \% \\\hline
	\end{tabular}

\begin{subfigure}{\textwidth}
	% CTI graph
	\begin{tikzpicture}
	    \begin{axis}
	        [
	        ymode=log,
	        log origin=infty,
	        xtick=data,
	        xtick style={draw=none},
	        x axis line style={draw=none},
	        minor tick num=1,
	        height=6cm,
	        width=\textwidth,
	        enlarge x limits=0.05,,
	        enlarge y limits={upper=0},
	        xlabel={Maximum Number of Pebbles},
	        xticklabels={7,8,9,10,11,12,13,14,15,16,17,18,29},
	        ybar,
	        axis y line*=left,
	        bar width=7pt,
	        legend style={at={(0.5,1.13)}, anchor=north,legend columns=-1},
	        ylabel={No. ctis},
	        x dir = reverse,
	        fill between/on layer={main},
	        ]
	        \legend{\cipdr cti-count, naive cti-count}
%	        \begin{filecontents}{gf2^5mult_29_129 cti-count.dat}
        	\pgfplotstableread{
	   			x y err
	   			7 0.9 0.6935416353759881
	   			8 1.7 0.09486832980505139
	   			9 1.2 0.06324555320336757
	   			10 1 0
	   			11 1 0
	   			12 1 0
	   			13 2.6 1.8044389709823938
	   			14 2.3333333333333335 1.7690759253434065
	   			15 2 1.7320508075688772
	   			16 1 0
	   			17 1.6666666666666667 0.693888666488711
	   			18 3 0
	   			20 4.9 1.131812705353673 
	   			% 29
	        }\cticount;
	        \errorbarplot{blue}{\cticount};
%	        \begin{filecontents}{gf2^5mult_29_129 naive cti-count.dat}
	        \pgfplotstableread{
			    x y err
			    7 6.3 0.09486832980505133
			    8 9.4 1.0178408519999578
			    9 7.5 0.15811388300841897
			    10 7.5 0.15811388300841897
			    11 7.5 0.15811388300841897
			    12 7.5 0.15811388300841897
			    13 7.5 0.15811388300841897
			    14 7.666666666666667 0.13608276348795423
			    15 7.666666666666667 0.1924500897298751
			    16 5 0
			    17 6 1
			    18 6 1
			    20 4.9 1.131812705353673 
			    % 29
	        }\ncticount;
	        \errorbarplot{red}{\ncticount};
	        
 	       	\defxcrunch{0.1}{0.15}
   		\end{axis}
    
		\drawxcrunch
	
	    \begin{axis}
	        [
	        ymode=log,
	        log origin=infty,
	        xtick=data,
	        xtick style={draw=none},
	        x axis line style={draw=none},
	        minor tick num=1,
	        height=6cm,
	        width=\textwidth,
	        enlarge x limits=0.05,,
	        enlarge y limits={upper=0},
	        axis y line*=right,
	        legend style={at={(0.5,1.0)}, anchor=north,legend columns=-1},
	        xticklabels={,,},
	        ylabel={Time (s)},
	        x dir = reverse,
	        fill between/on layer={main},
	        ]
	        \legend{\cipdr cti-time, naive cti-time}
%	        \begin{filecontents}{gf2^5mult_29_129 cti-time.dat}
        	\pgfplotstableread{
	            x y err
	            7 11.3303083389 11.993091054157082
	            8 449.8725357669 141.7051561349265
	            9 328.4225072991 103.05765366562608
	            10 156.49523181759997 35.80280399062704
	            11 149.0131219511 28.727888702395248
	            12 86.2631789925 24.07833738429544
	            13 38.3670494976 9.504794614178326
	            14 17.299639153500003 8.218879423738036
	            15 7.110512637249999 2.754842071407898
	            16 3.342679417333333 2.836740643489416
	            17 2.454383569 1.3683369065562152
	            18 4.3024822965 0.2217436045000003
	            20 3.5391886453 0.5935547533664379 
	            % 29
	        }\ctitime;
        
	        \dotplot{blue}{\ctitime};
	        \addplot [name path=upper,draw=none]
	        table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\ctitime};
	        \addplot [name path=lower,draw=none] 
	        table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\ctitime};
	        \filldevplot{blue}
%	        \begin{filecontents}{gf2^5mult_29_129 naive cti-time.dat}
        	\pgfplotstableread{
	            x y err
	            7 18.0574196793 0.8316385357226574
	            8 274.5368143227 103.51759354474454
	            9 163.36035096260002 116.0287193106663
	            10 121.7796687272 57.54074367793935
	            11 74.4429681653 60.11911841804375
	            12 55.3292894442 50.20665306447309
	            13 33.383235055200004 23.309240683902196
	            14 14.597230637166666 5.900603676090597
	            15 9.133631801333335 1.5034263596489605
	            16 6.1449246005 0.44350272849999994
	            17 5.6213646725 0.022048734499999778
	            18 5.9116867504999995 1.1366761865000004
	            20 3.5431552921000007 0.5957758472520305 
	            % 29
	        }\nctitime;
        
	        \dotplot{red}{\nctitime}
	        \addplot [name path=upper,draw=none]
	        table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\nctitime};
	        \addplot [name path=lower,draw=none] 
	        table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\nctitime};
	        \linedevplot{red}
        \end{axis}
	    %\caption{Statistics for gf2^5mult_29_129 experiment.}
	\end{tikzpicture}
	\caption{
		A comparison between the number of counterexamples found in the major
		iteration (cti-count) on the left axis and the total runtime (cti-time)
		on the right axis.
	}
	\label{fig:pebbling:constrain:gf2-129:cti}
	\end{subfigure}

	\begin{subfigure}{\textwidth}
		\centering
	% Incremental times
	\begin{tikzpicture}		
		\begin{axis}
			[
			xtick=data,
			xtick style={draw=none},
			minor tick num=1,
			height=4cm,
			width=0.8\textwidth,
			enlarge x limits=0.05,,
			enlarge y limits={upper=0},
			xlabel={Maximum Number of Pebbles},
%			axis y line*=left,
			legend style={at={(0.5,1.23)}, anchor=north,legend columns=-1},
			ylabel={Time (s)},
			x dir = reverse,
			fill between/on layer={main},
			]
			\legend{\cipdr inc-time, naive inc-time}
%			\begin{filecontents}{gf2^5mult_29_129 inc-time (constrain).dat}
			\pgfplotstableread{
				x y err
				7 1.9392231881999997 0.2251352277988565
				8 1.2945254886000002 0.13983417873148157
				9 0.7289119802 0.07132842559883489
				10 0.42779848740000004 0.07231976141992544
				11 0.2078407285 0.042024061621613526
				12 0.1053225023 0.03376558357791847
				13 0.05209678720000001 0.025414614937018434
				14 0.04713656166666667 0.014592675172891737
				15 0.044189242999999996 0.010458119966187588
				16 0.04322967366666666 0.003041364270205102
				17 0.039145995999999995 0.0017789814906155345
				18 0.0390679715 0.00028767949999999876
			}\inctime
			\dotplot{blue}{\inctime};
			\addplot [name path=upper,draw=none]
				table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\inctime};
			\addplot [name path=lower,draw=none] 
				table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\inctime};
			\filldevplot{blue}
%			\begin{filecontents}{gf2^5mult_29_129 naive inc-time (constrain).dat}
			\pgfplotstableread{
				x y err
				7 0.0661744769 0.0014407403165031137
				8 0.06504124550000001 0.0017091838637540006
				9 0.06419313630000001 0.000968760084887076
				10 0.0634011717 0.0011390990922297373
				11 0.0627038834 0.0011187449181320301
				12 0.0628574298 0.0007011081008758623
				13 0.062029324 0.0003845119471938429
				14 0.06225605666666667 0.0013711092861033692
				15 0.06151670100000001 0.0003074639216862162
				16 0.061838847 5.662999999999502e-06
				17 0.061301362 0.0004085779999999997
				18 0.061370751 0.00016926899999999967
			}\ninctime
			\dotplot{red}{\ninctime};
			\addplot [name path=upper,draw=none]
				table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\ninctime};
			\addplot [name path=lower,draw=none] 
				table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\ninctime};
			\linedevplot{red}
		\end{axis}
	\end{tikzpicture}
	\caption{
		The amount of the runtime that was spent on copying clauses to the
		constrained instance denoted on the x-axis. This number is already included
		in the times of the upper graph. 	
	}
	\label{fig:pebbling:constrain:gf2-129:inc}
	\end{subfigure}
	\caption{
	    Statistics for the constraining \texttt{gf2\^{}5mult\_29\_129} experiment,
	    averaged over each repetition.
	    On constraint 29, the algorithm found a trace with 19 pebbles, so it could continue with constraint 18 afterwards.
	}
    \label{fig:pebbling:constrain:gf2-129}
\end{figure}

{
\newcommand{\plotheight}{6cm}
% Obligation graph
\begin{figure}[h]
\centering
\begin{subfigure}{\textwidth}
\begin{tikzpicture}
    \begin{axis}
    [
        ymode=log,
        log origin=infty,
        xtick=data,
        xtick style={draw=none},
        x axis line style={draw=none},
        minor tick num=1,
        height=\plotheight,
        width=\textwidth,
        enlarge x limits=0.05,,
        enlarge y limits={upper=0},
        xlabel={Maximum Number of Pebbles},
        xticklabels={7,8,9,10,11,12,13,14,15,16,17,18,29},
        ybar,
        axis y line*=left,
        bar width=7pt,
        legend style={at={(0.5,1.17)}, anchor=north,legend columns=-1},
        ylabel={No. obligations},
        x dir = reverse,
        fill between/on layer={main},
    ]
        \legend{\cipdr obligation-count, naive obligation-count}
%        \begin{filecontents}{gf2^5mult_29_129 obligation-count.dat}
        \pgfplotstableread{
		    x y err
		    7 4.9 6.580349534789167
		    8 225.8 23.933324048280465
		    9 184.2 36.74920407301361
		    10 132.8 16.22294671137152
		    11 124.4 11.34795135696307
		    12 99.5 14.880356178532825
		    13 83.7 24.37435127341854
		    14 58.333333333333336 19.26472500789019
		    15 43.75 24.94024107742345
		    16 29.333333333333332 6.938886664887109
		    17 40.333333333333336 11.767815493178055
		    18 54.5 4.4860896112315904
		    20 140.7 8.404106139263115
		    % 29
        }\oblcount
        \errorbarplot{blue}{\oblcount};
%        \begin{filecontents}{gf2^5mult_29_129 naive obligation-count.dat}
		\pgfplotstableread{
			x y err
			7 22.2 0.5513619500836088
			8 382.7 58.05298441940776
			9 307.9 63.7463802893937
			10 282.6 41.85924031799908
			11 235.4 49.22820329851578
			12 215.6 38.344960555462826
			13 199.2 29.812816036060735
			14 180.33333333333334 17.93868156516237
			15 166 4.96655480858378
			16 157.5 8.492643875731515
			17 149 6
			18 149 11
			20 140.7 8.404106139263115
			% 29
        }\noblcount
        \errorbarplot{red}{\noblcount};
        
       	\defxcrunch{0.1}{0.15}
	\end{axis}
  
	\drawxcrunch

    \begin{axis}
        [
        ymode=log,
        log origin=infty,
        xtick=data,
        xtick style={draw=none},
        x axis line style={draw=none},
        minor tick num=1,
        height=\plotheight,
        width=\textwidth,
        enlarge x limits=0.05,,
        enlarge y limits={upper=0},
        axis y line*=right,
        legend style={at={(0.5,1.04)}, anchor=north,legend columns=-1},
        xticklabels={,,},
        ylabel={Time (s)},
        x dir = reverse,
        fill between/on layer={main},
        ]
        \legend{\cipdr obligation-time, naive obligation-time}
%        \begin{filecontents}{gf2^5mult_29_129 obligation-time.dat}
		\pgfplotstableread{
			x y err
			7 9.1443559441 11.516491513096188
			8 448.2848744407 141.524672208424
			9 327.8884866038 103.18035059008965
			10 156.3272832592 35.802316619861344
			11 148.87998889129997 28.731149509429
			12 86.14657556519998 24.077323716769666
			13 38.17661341670001 9.527815717648114
			14 17.138407675833335 8.265400797404377
			15 6.979195838749998 2.6706824695978577
			16 3.266981703666667 2.8325422699129876
			17 2.342413442666667 1.3213011960532788
			18 4.125727629 0.2202609790000003
			20 3.3648410794999997 0.5474155227680557
			% 29
        }\obltime
        \dotplot{blue}{\obltime};
        \addplot [name path=upper,draw=none]
        	table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\obltime};
        \addplot [name path=lower,draw=none] 
        	table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\obltime};
        \filldevplot{blue}
%        \begin{filecontents}{gf2^5mult_29_129 naive obligation-time.dat}
		\pgfplotstableread{
			x y err
			7 17.9292683475 0.8288775442678362
			8 273.85166012850004 103.36541812109462
			9 162.97179129079998 115.96556687842686
			10 121.40764635219996 57.49655759898945
			11 74.13065282499996 60.077010889342496
			12 55.03911184350001 50.18143767832271
			13 33.097752196699986 23.286803508764418
			14 14.32867533016666 5.890046035925796
			15 8.870674912333333 1.50088517870214
			16 5.9670091015 0.4413040654999998
			17 5.410062137999997 0.0594758320000035
			18 5.697339874500001 1.0867411435000025
			20 3.368120019700001 0.5494901780153068
			% 29
        }\nobltime
        \dotplot{red}{\nobltime};
        \addplot [name path=upper,draw=none]
        	table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\nobltime};
        \addplot [name path=lower,draw=none] 
        	table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\nobltime};
        \linedevplot{red}
        
    \end{axis}
    %\caption{Statistics for gf2^5mult_29_129 experiment.}
    
	\end{tikzpicture}
	\caption{
	    Left axis: total number of obligations (obligation-count)
	    handled by the minor iteration. Right axis: the time spent on
	    them (obligation-time).
	}\label{fig:pebbling:constrain:gf2-129:obl}
\end{subfigure}

\begin{subfigure}{\textwidth}
% SAT-call graph
\begin{tikzpicture}
    \begin{axis}
        [
        ymode=log,
        log origin=infty,
        xtick=data,
        xtick style={draw=none},
        x axis line style={draw=none},
        minor tick num=1,
        height=\plotheight,
        width=\textwidth,
        enlarge x limits=0.05,,
        enlarge y limits={upper=0},
        xlabel={Maximum Number of Pebbles},
        xticklabels={7,8,9,10,11,12,13,14,15,16,17,18,29},
        ybar,
        axis y line*=left,
        bar width=7pt,
        legend style={at={(0.5,1.13)}, anchor=north,legend columns=-1},
        ylabel={No. \sat-queries},
        x dir = reverse,
        fill between/on layer={main},
        ]
        \legend{\cipdr sat-count, naive sat-count}
%        \begin{filecontents}{gf2^5mult_29_129 sat-count.dat}
		\pgfplotstableread{
			x y err
			7 2702.5 1772.8318095634454
			8 37966.2 6206.579294909556
			9 31591.1 7358.417362517567
			10 19366.3 3530.3223095065982
			11 19294.9 2850.439952182821
			12 12791.3 2499.79338526207
			13 7067 1456.5591646067796
			14 3565.5 1113.7061439176853
			15 1742.75 962.4811767639926
			16 800.3333333333334 572.731208366575
			17 886 488.1768805122449
			18 1538 97
			20 2863.2 270.5053862680002
			% 29
        }\satcount
        \errorbarplot{blue}{\satcount}
%        \begin{filecontents}{gf2^5mult_29_129 naive sat-count.dat}
		\pgfplotstableread{
			x y err
			7 3256.25 1374.8614850685867
			8 37229.6 8943.965198836588
			9 27058 9891.858121707974
			10 19406.3 5357.4464537221465
			11 16409.85 6535.121273635631
			12 12014.25 5278.0554637219375
			13 7796.8 2948.691203228985
			14 4651.25 1613.3037935269147
			15 2980.714285714286 1621.200207778985
			16 2036.4 1584.0789475275528
			17 2004 1421.9836848571788
			18 2625.5 1126.664574085828
			20 2863.2 270.5053271194488
			% 29
        }\nsatcount
        \errorbarplot{red}{\nsatcount}
        
       	\defxcrunch{0.1}{0.15}
	\end{axis}
	
	\drawxcrunch

    \begin{axis}
    [
        ymode=log,
        log origin=infty,
        xtick=data,
        xtick style={draw=none},
        x axis line style={draw=none},
        minor tick num=1,
        height=\plotheight,
        width=\textwidth,
        enlarge x limits=0.05,,
        enlarge y limits={upper=0},
        axis y line*=right,
        legend style={at={(0.5,1.0)}, anchor=north,legend columns=-1},
        xticklabels={,,},
        ylabel={Time (s)},
        x dir = reverse,
        fill between/on layer={main},
    ]
        \legend{\cipdr sat-time, naive sat-time}
%        \begin{filecontents}{gf2^5mult_29_129 sat-time.dat}
		\pgfplotstableread{
			x y err
			7 7.646665180299995 4.890335441124495
			8 290.01735852729956 114.34362838472724
			9 196.8747273855996 72.05894782875521
			10 77.56368204069989 21.41881059830343
			11 69.26199965369996 16.400692324469397
			12 34.29657248590003 13.339876036772376
			13 12.017839175699986 3.647605020915823
			14 4.970332971833337 2.7735088306818545
			15 1.8958567549999978 0.8401928992540922
			16 0.8998208986666669 0.7307229950232554
			17 0.7130369359999998 0.38880851865168375
			18 1.2360456754999984 0.0720052954999999
			20 1.4791777195999996 0.19711996989487146
			% 29
        }\sattime
        \dotplot{blue}{\sattime};
        \addplot [name path=upper,draw=none]
            table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\sattime};
        \addplot [name path=lower,draw=none] 
            table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\sattime};
        \filldevplot{blue}
%        \begin{filecontents}{gf2^5mult_29_129 naive sat-time.dat}
		\pgfplotstableread{
			x y err
			7 6.232513947249998 3.7415643733830617
			8 215.26780271834974 117.52987363163547
			9 142.12913690279987 92.37563218490578
			10 67.83537257049996 28.33741714754384
			11 51.370885470899985 29.563407835291954
			12 28.79055250595001 19.1224665045539
			13 12.191156475099993 6.816469323755204
			14 4.792455350833338 2.308447059802189
			15 2.3654187565714264 0.8694456341335961
			16 1.4385386141999994 0.8747970285608669
			17 1.267048712399999 0.7429909340452209
			18 1.7083535249999988 0.5301233964602274
			20 1.48034046715 0.19816306182291082
			% 29
        }\nsattime
        \dotplot{red}{\nsattime};
        \addplot [name path=upper,draw=none]
        	table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\nsattime};
        \addplot [name path=lower,draw=none] 
        	table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\nsattime};
        \linedevplot{red}
    \end{axis}

\end{tikzpicture}
\caption{
    Left axis: the total number of calls to the \sat-solver (sat-count). Right axis: the total time spent waiting on the \sat-solver (sat-time..
}\label{fig:pebbling:constrain:gf2-129:sat}
\end{subfigure}
\caption{
	Constraining \texttt{gf2\^{}5mult\_29\_129} experiment (10 repetitions). Left axis: the number of counterexamples (cti-count) found in the major iteration. Right axis: the total runtime (cti-time).
	On constraint 23, the algorithm found a trace with 18 pebbles, so it could continue with 17 afterwards.
}
\label{fig:pebbling:constrain:gf2-129:oblsat}
\end{figure}
}


==> sections/experiments/results/old/new-results.tex <==
\begin{figure}
\centering
\begin{vsplot}{\cipdr, naive \cipdr}{
    \texttt{mod5d1},
    \texttt{gf2\^{}3mult\_11\_47},
    \texttt{ham3tc},
}
    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit
    ] coordinates {
    	(\texttt{mod5d1}, 0.690) +- (0, 0.006)
    	(\texttt{gf2\^{}3mult\_11\_47}, 2.101) +- (0, 0.213)
    	(\texttt{ham3tc}, 0.022) +- (0, 0.000)
    };

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit
    ] coordinates {
    	(\texttt{mod5d1}, 1.247) +- (0, 0.016)
    	(\texttt{gf2\^{}3mult\_11\_47}, 2.568) +- (0, 0.030)
    	(\texttt{ham3tc}, 0.022) +- (0, 0.000)
    };
\end{vsplot}
\end{figure}

\begin{figure}
\centering
\begin{vsplot}{\cipdr, naive \cipdr}{
    \texttt{mod5d1},
    \texttt{gf2\^{}3mult\_11\_47},
    \texttt{4b15g\_1},
    \texttt{gf2\^{}4mult\_19\_83},
}
    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit
    ] coordinates {
    	(\texttt{mod5d1}, 0.690) +- (0, 0.006)
    	(\texttt{gf2\^{}3mult\_11\_47}, 2.101) +- (0, 0.213)
    	(\texttt{4b15g\_1}, 7.010) +- (0, 0.217)
    	(\texttt{gf2\^{}4mult\_19\_83}, 108.961) +- (0, 18.739)
    };

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit
    ] coordinates {
    	(\texttt{mod5d1}, 1.247) +- (0, 0.016)
    	(\texttt{gf2\^{}3mult\_11\_47}, 2.568) +- (0, 0.030)
    	(\texttt{4b15g\_1}, 28.395) +- (0, 2.289)
    	(\texttt{gf2\^{}4mult\_19\_83}, 23.267) +- (0, 7.848)
    };
\end{vsplot}
\end{figure}

\begin{figure}
\centering
\begin{vsplot}{\cipdr, naive \cipdr}{
    \texttt{5bitadder},
    \texttt{5mod5tc},
    \texttt{gf2\^{}5mult\_29\_129},
    \texttt{ham7tc},
}
    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit
    ] coordinates {
    	(\texttt{5bitadder}, 890.704) +- (0, 177.617)
    	(\texttt{5mod5tc}, 1487.176) +- (0, 149.927)
    	(\texttt{gf2\^{}5mult\_29\_129}, 1258.402) +- (0, 216.143)
    	(\texttt{ham7tc}, 160.033) +- (0, 94.802)
    };

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit
    ] coordinates {
    	(\texttt{5bitadder}, 1669.661) +- (0, 240.941)
    	(\texttt{5mod5tc}, 1576.194) +- (0, 68.088)
    	(\texttt{gf2\^{}5mult\_29\_129}, 974.229) +- (0, 243.754)
    	(\texttt{ham7tc}, 571.523) +- (0, 91.298)
    };
\end{vsplot}
\end{figure}


==> sections/experiments/results/old/pebbling-results.tex <==
\begin{figure}
    \centering 
    \begin{vsplot}{\cipdr, naive \cipdr, \bmc}{
        \texttt{mod5d1},
        \texttt{gf2\^{}3mult\_11\_47}
    }
        \addplot+[
            error bars/.cd,
            y dir=both,
            y explicit
        ] coordinates {
          (\texttt{mod5d1}, 0.850) +- (0, 0.009)
          (\texttt{gf2\^{}3mult\_11\_47}, 1.968) +- (0, 0.151)
        };
         
        \addplot+[
            error bars/.cd,
            y dir=both,
            y explicit
        ] coordinates{
          (\texttt{mod5d1}, 1.253) +- (0, 0.002)
          (\texttt{gf2\^{}3mult\_11\_47}, 2.351) +- (0, 0.144)
        };
    \end{vsplot}
    
    % \columnbreak
    % \hfill \texttt{mod5d1}: 120.534
    
    % \hfill \texttt{gf2\^{}3mult\_11\_47}: 121.676
    \caption{Short experiments without \bmc comparison.} \label{fig:exp:nobmc}
\end{figure}

\begin{figure}
    \begin{vsplot}{\cipdr, naive \cipdr, \bmc}{
        \texttt{mod5d1},
        \texttt{gf2\^{}3mult\_11\_47},
        \texttt{4b15g\_1}, \texttt{gf\^{}4mult\_19\_83}
    }
        \addplot+[
            error bars/.cd,
            y dir=both,
            y explicit
        ] coordinates{
            (\texttt{mod5d1}, 0.850) +- (0, 0.009)
            (\texttt{gf2\^{}3mult\_11\_47}, 1.968) +- (0, 0.151)
            (\texttt{4b15g\_1}, 7.260) +- (0, 1.148) 
            (\texttt{gf\^{}4mult\_19\_83}, 44.358) +- (0, 4.611) 
        };
        \addplot+[
            error bars/.cd,
            y dir=both,
            y explicit
        ] coordinates{
            (\texttt{mod5d1}, 1.253) +- (0, 0.002)
            (\texttt{gf2\^{}3mult\_11\_47}, 2.351) +- (0, 0.144)
            (\texttt{4b15g\_1}, 28.533) +- (0, 0.067) 
            (\texttt{gf\^{}4mult\_19\_83}, 17.440) +- (0, 3.334) 
        };
        \addplot+[
            error bars/.cd,
            y dir=both,
            y explicit
        ] coordinates{
            (\texttt{mod5d1}, 120.534)
            (\texttt{gf2\^{}3mult\_11\_47}, 121.676)
            (\texttt{4b15g\_1}, 121.748)
            (\texttt{gf\^{}4mult\_19\_83}, 129.573)
        };
    \end{vsplot}
    % \columnbreak
    % \hfill \texttt{4b15g\_1}: 121.748
    
    % \hfill \texttt{gf\^{}4mult\_19\_83}: 129.573
    \caption{Short experiments with \bmc comparison.} \label{fig:exp:1}
\end{figure}

\begin{figure}
    \begin{vsplot}{\cipdr, naive \cipdr, \bmc}{
        \texttt{5bitadder}, \texttt{5mod5tc}, \texttt{gf2\^{}5mult\_29\_129}
    }
        \addplot+[
            error bars/.cd,
            y dir=both,
            y explicit
        ] coordinates{
            (\texttt{5bitadder}, 243.517) +- (0, 39.982) 
            (\texttt{5mod5tc}, 306.205) +- (0, 11.215)
            (\texttt{gf2\^{}5mult\_29\_129}, 343.931) +- (0, 62.980)
        };
        \addplot+[
            error bars/.cd,
            y dir=both,
            y explicit
        ] coordinates{
            (\texttt{5bitadder}, 343.743) +- (0, 32.728) 
            (\texttt{5mod5tc}, 384.828) +- (0, 9.878)
            (\texttt{gf2\^{}5mult\_29\_129}, 270.859) +- (0, 30.052)
        };
        \addplot+[
            error bars/.cd,
            y dir=both,
            y explicit
        ] coordinates{
            (\texttt{5bitadder}, 145.708)
            (\texttt{5mod5tc}, 124.481)
            (\texttt{gf2\^{}5mult\_29\_129}, 240.666)
        };
    \end{vsplot}
    
    % \columnbreak
    % \hfill \texttt{5bitadder}: 145.708
    
    % \hfill \texttt{5mod5tc}: 124.481
    
    % \hfill \texttt{gf2\^{}5mult\_29\_129}: 240.666
    \caption{Long experiments with \bmc comparison.} \label{fig:exp:2}
\end{figure}



==> sections/experiments/results/old/results-bin.tex <==
% only slower on gf2 models
\begin{figure}
% \centering
\begin{vsplot}{binary search \ipdr, naive binary search \ipdr}{
    % a,
    b,
    c,
    d,
    e,
    f,
    g,
    h,
    i,
    j,
}
    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit
    ] coordinates {
			% (0, 0.005) +- (0, 0.000)	% rd32
			(b, 0.025) +- (0, 0.000)	% ham3tc
			(c, 0.628) +- (0, 0.018)	% mod5d1
			(d, 2.191) +- (0, 0.310)	% gf2\^{}3mult\_11\_47
			(e, 9.880) +- (0, 2.130)	% 4b15g\_1
			(f, 67.429) +- (0, 39.057)	% gf2\^{}4mult\_19\_83
			(g, 1106.458) +- (0, 538.147)	% 5mod5tc
			(h, 528.734) +- (0, 196.339)	% gf2\^{}5mult\_29\_129
			(i, 24.970) +- (0, 10.087)	% ham7tc
			(j, 395.247) +- (0, 148.613)	% 5bitadder

    };

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit,
    ] coordinates {
			% (0, 0.005) +- (0, 0.000)	% rd32
			(b, 0.025) +- (0, 0.000)	% ham3tc
			(c, 0.677) +- (0, 0.066)	% mod5d1
			(d, 1.508) +- (0, 0.246)	% gf2\^{}3mult\_11\_47
			(e, 18.334) +- (0, 3.933)	% 4b15g\_1
			(f, 18.907) +- (0, 12.187)	% gf2\^{}4mult\_19\_83
			(g, 1283.805) +- (0, 606.028)	% 5mod5tc
			(h, 478.353) +- (0, 198.222)	% gf2\^{}5mult\_29\_129
			(i, 188.639) +- (0, 184.351)	% ham7tc
			(j, 499.284) +- (0, 133.449)	% 5bitadder
    };

\end{vsplot}
\caption{ (partial min core) binary search v1 results \\
	a = \texttt{rd32},
	b = \texttt{ham3tc},
	c = \texttt{mod5d1},
  d = \texttt{gf2\^{}3mult\_11\_47},
  e = \texttt{4b15g\_1},
  f = \texttt{gf2\^{}4mult\_19\_83},
  g = \texttt{5mod5tc},
  h = \texttt{gf2\^{}5mult\_29\_129},
  i = \texttt{ham7tc},
  j = \texttt{5bitadder},
}
\end{figure}

\begin{figure}
% \centering
\begin{vsplot}{binary search \ipdr, naive binary search \ipdr}{
    % a,
    b,
    c,
    d,
    e,
    f,
    g,
    h,
    i,
    j,
}
    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit
    ] coordinates {
        % (0, 0.005) +- (0, 0.000)	% rd32
        (b, 0.025) +- (0, 0.000)	% ham3tc
        (c, 0.631) +- (0, 0.017)	% mod5d1
        (d, 2.159) +- (0, 0.086)	% gf2\^{}3mult\_11\_47
        (e, 9.333) +- (0, 2.227)	% 4b15g\_1
        (f, 71.882) +- (0, 33.024)	% gf2\^{}4mult\_19\_83
        (g, 595.840) +- (0, 682.215)	% 5mod5tc
        (h, 523.172) +- (0, 142.971)	% gf2\^{}5mult\_29\_129
        (i, 28.673) +- (0, 14.160)	% ham7tc
        (j, 305.039) +- (0, 116.698)	% 5bitadder
    };

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit,
    ] coordinates {
        % (0, 0.005) +- (0, 0.000)	% rd32
        (b, 0.025) +- (0, 0.000)	% ham3tc
        (c, 0.683) +- (0, 0.062)	% mod5d1
        (d, 1.643) +- (0, 0.112)	% gf2\^{}3mult\_11\_47
        (e, 17.123) +- (0, 3.384)	% 4b15g\_1
        (f, 25.572) +- (0, 18.763)	% gf2\^{}4mult\_19\_83
        (g, 716.151) +- (0, 754.209)	% 5mod5tc
        (h, 527.323) +- (0, 118.696)	% gf2\^{}5mult\_29\_129
        (i, 164.083) +- (0, 164.698)	% ham7tc
        (j, 692.735) +- (0, 88.123)	% 5bitadder
    };

\end{vsplot}
\caption{ binary search v1 results \\
	a = \texttt{rd32},
	b = \texttt{ham3tc},
	c = \texttt{mod5d1},
  d = \texttt{gf2\^{}3mult\_11\_47},
  e = \texttt{4b15g\_1},
  f = \texttt{gf2\^{}4mult\_19\_83},
  g = \texttt{5mod5tc},
  h = \texttt{gf2\^{}5mult\_29\_129},
  i = \texttt{ham7tc},
  j = \texttt{5bitadder},
}
\end{figure}



==> sections/experiments/results/old/results-full.tex <==
\message{
    Deprecated Results: the z3-spacer results in results-full.tex are improved
    by results-full2.tex
}
\begin{figure}
% \centering
\begin{vsplot}{\cipdr, naive \cipdr, z3-spacer}{
    a,
    b,
    c,
    d,
    e,
    f,
    g,
    h,
    i,
}
    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit
    ] coordinates {
        (a, 0.690) +- (0, 0.006)      % mod5d1
        (b, 2.101) +- (0, 0.213)      % gf2\^{}3mult\_11\_47
        (c, 0.022) +- (0, 0.000)      % ham3tc
        (d, 7.010) +- (0, 0.217)      % 4b15g\_1
        (e, 108.961) +- (0, 18.739)   % gf2\^{}4mult\_19\_83
        (f, 890.704) +- (0, 177.617)	% 5bitadder
        (g, 1487.176) +- (0, 149.927)	% 5mod5tc
        (h, 1258.402) +- (0, 216.143)	% gf2\^{}5mult\_29\_129
        (i, 160.033) +- (0, 94.802)	  % ham7tc
    };

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit,
    ] coordinates {
    	(a, 1.247) +- (0, 0.016)      % mod5d1
    	(b, 2.568) +- (0, 0.030)      % gf2\^{}3mult\_11\_47
    	(c, 0.022) +- (0, 0.000)      % ham3tc
    	(d, 28.395) +- (0, 2.289)     % 4b15g\_1
    	(e, 23.267) +- (0, 7.848)     % gf2\^{}4mult\_19\_83
    	(f, 1669.661) +- (0, 240.941)	% 5bitadder
    	(g, 1576.194) +- (0, 68.088)	% 5mod5tc
    	(h, 974.229) +- (0, 243.754)	% gf2\^{}5mult\_29\_129
    	(i, 571.523) +- (0, 91.298)	  % ham7tc
    };

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit,
    ] coordinates {
        (a, 12.650) +- (0, 1.344)    % mod5d1
        (b, 22.446) +- (0, 5.363)    % gf2\^{}3mult\_11\_47
        (c, 1.063) +- (0, 0.113)     % ham3tc
        (d, 308.462) +- (0, 139.842) % 4b15g\_1
        (e, 906.987) +- (0, 218.677) % gf2\^{}4mult\_19\_83
    };
\end{vsplot}
\caption{
	a = \texttt{mod5d1},
	b = \texttt{gf2\^{}3mult\_11\_47},
	c = \texttt{ham3tc},
  d = \texttt{4b15g\_1},
  e = \texttt{gf2\^{}4mult\_19\_83},
  f = \texttt{5bitadder},
  g = \texttt{5mod5tc},
  h = \texttt{gf2\^{}5mult\_29\_129},
  i = \texttt{ham7tc},
}
\end{figure}



==> sections/experiments/results/old/results-full2.tex <==
\begin{figure}
% \centering
\begin{vsplot}{\cipdr, naive \cipdr, z3-spacer}{
    a,
    b,
    c,
    d,
    e,
    f,
    g,
    h,
    i,
}
    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit
    ] coordinates {
        (a, 0.690) +- (0, 0.006)      % mod5d1
        (b, 2.101) +- (0, 0.213)      % gf2\^{}3mult\_11\_47
        (c, 0.022) +- (0, 0.000)      % ham3tc
        (d, 7.010) +- (0, 0.217)      % 4b15g\_1
        (e, 108.961) +- (0, 18.739)   % gf2\^{}4mult\_19\_83
        (f, 890.704) +- (0, 177.617)	% 5bitadder
        (g, 1487.176) +- (0, 149.927)	% 5mod5tc
        (h, 1258.402) +- (0, 216.143)	% gf2\^{}5mult\_29\_129
        (i, 160.033) +- (0, 94.802)	  % ham7tc
    };

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit,
    ] coordinates {
    	(a, 1.247) +- (0, 0.016)      % mod5d1
    	(b, 2.568) +- (0, 0.030)      % gf2\^{}3mult\_11\_47
    	(c, 0.022) +- (0, 0.000)      % ham3tc
    	(d, 28.395) +- (0, 2.289)     % 4b15g\_1
    	(e, 23.267) +- (0, 7.848)     % gf2\^{}4mult\_19\_83
    	(f, 1669.661) +- (0, 240.941)	% 5bitadder
    	(g, 1576.194) +- (0, 68.088)	% 5mod5tc
    	(h, 974.229) +- (0, 243.754)	% gf2\^{}5mult\_29\_129
    	(i, 571.523) +- (0, 91.298)	  % ham7tc
    };

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit,
    ] coordinates {
        (a, 2.951) +- (0, 0.235)    % mod5d1
        (b, 2.884) +- (0, 0.623)    % gf2\^{}3mult\_11\_47
        (c, 0.214) +- (0, 0.013)    % ham3tc
        (d, 14.348) +- (0, 3.357)   % 4b15g\_1
        (e, 35.733) +- (0, 9.106)   % gf2\^{}4mult\_19\_83
        (f, 0) +- (0, 0)            % 5bitadder
        (g, 411.649) +- (0, 40.772) % 5mod5tc
        (h, 418.718) +- (0, 69.834) % gf2\^{}5mult\_29\_129
        (i, 106.773) +- (0, 24.068) % ham7tc
        % (\texttt{rd32}, 0.176) +- (0, 0.007) % rd32
    };
\end{vsplot}
\caption{
	a = \texttt{mod5d1},
	b = \texttt{gf2\^{}3mult\_11\_47},
	c = \texttt{ham3tc},
  d = \texttt{4b15g\_1},
  e = \texttt{gf2\^{}4mult\_19\_83},
  f = \texttt{5bitadder},
  g = \texttt{5mod5tc},
  h = \texttt{gf2\^{}5mult\_29\_129},
  i = \texttt{ham7tc},
} \label{experiments:pebbling:results}
\end{figure}



==> sections/experiments/results/old/results-full3.tex <==
\begin{figure}
% \centering
\begin{vsplot}{\cipdr, naive \cipdr, z3-spacer}{
    % a,
    b,
    c,
    d,
    e,
    f,
    g,
    h,
    i,
    j,
}
    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit
    ] coordinates {
        % naive cipdr
                                      % all 0 seed?
        % (a, 0.006) +- (0, 0.002)	    % rd32
        (b, 0.025) +- (0, 0.001)	    % ham3tc
        (c, 0.752) +- (0, 0.018)	    % mod5d1
        (d, 2.160) +- (0, 0.144)	    % gf2\^{}3mult\_11\_47
        (e, 10.206) +- (0, 1.977)	    % 4b15g\_1
        (f, 101.118) +- (0, 12.279)	  % gf2\^{}4mult\_19\_83
        (g, 1578.834) +- (0, 121.287)	% 5mod5tc
        (h, 1284.055) +- (0, 351.351)	% gf2\^{}5mult\_29\_129
        (i, 165.732) +- (0, 98.251)	  % ham7tc
        (j, 902.333) +- (0, 0.000)	% 5bitadder (1 sample)
    };

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit,
    ] coordinates {
        % naive cipdr
        % (0, 0.005) +- (0, 0.000)	    % rd32
        (b, 0.025) +- (0, 0.000)	    % ham3tc
        (c, 1.321) +- (0, 0.035)	    % mod5d1
        (d, 2.716) +- (0, 0.390)	    % gf2\^{}3mult\_11\_47
        (e, 37.784) +- (0, 3.808)	    % 4b15g\_1
        (f, 58.676) +- (0, 13.872)	  % gf2\^{}4mult\_19\_83
        (g, 2246.857) +- (0, 76.189)	% 5mod5tc
        (h, 1021.491) +- (0, 157.994)	% gf2\^{}5mult\_29\_129
        (i, 561.574) +- (0, 56.444)	  % ham7tc
        (j, 1470.711) +- (0, 0.000)	    % 5bitadder (1 sample)
    };

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit,
    ] coordinates {
        % z3-spacer
        % (a, 0) +- (0,0)             % rd32
        (b, 0.214) +- (0, 0.013)    % ham3tc
        (c, 2.951) +- (0, 0.235)    % mod5d1
        (d, 2.884) +- (0, 0.623)    % gf2\^{}3mult\_11\_47
        (e, 14.348) +- (0, 3.357)   % 4b15g\_1
        (f, 35.733) +- (0, 9.106)   % gf2\^{}4mult\_19\_83
        (g, 411.649) +- (0, 40.772) % 5mod5tc
        (h, 418.718) +- (0, 69.834) % gf2\^{}5mult\_29\_129
        (i, 106.773) +- (0, 24.068) % ham7tc
        (j, 0) +- (0, 0)            % 5bitadder

        % (a, 2.951) +- (0, 0.235)    % mod5d1
        % (b, 2.884) +- (0, 0.623)    % gf2\^{}3mult\_11\_47
        % (c, 0.214) +- (0, 0.013)    % ham3tc
        % (d, 14.348) +- (0, 3.357)   % 4b15g\_1
        % (e, 35.733) +- (0, 9.106)   % gf2\^{}4mult\_19\_83
        % (f, 0) +- (0, 0)            % 5bitadder
        % (g, 411.649) +- (0, 40.772) % 5mod5tc
        % (h, 418.718) +- (0, 69.834) % gf2\^{}5mult\_29\_129
        % (i, 106.773) +- (0, 24.068) % ham7tc
        % (\texttt{rd32}, 0.176) +- (0, 0.007) % rd32
    };
\end{vsplot}
\caption{ With UNSAT-core in MIC disabled.
	a = \texttt{rd32},
	b = \texttt{ham3tc},
	c = \texttt{mod5d1},
  d = \texttt{gf2\^{}3mult\_11\_47},
  e = \texttt{4b15g\_1},
  f = \texttt{gf2\^{}4mult\_19\_83},
  g = \texttt{5mod5tc},
  h = \texttt{gf2\^{}5mult\_29\_129},
  i = \texttt{ham7tc},
  j = \texttt{5bitadder},
}
\end{figure}

\begin{figure}
% \centering
\begin{vsplotfour}
{core \cipdr, nocore \cipdr, core naive \cipdr, nocore naive \cipdr}
{
    % a,
    b,
    c,
    d,
    e,
    f,
    g,
    h,
    i,
    j,
}
    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit
    ] coordinates {
        % core
        (b, 0.022) +- (0, 0.000)      % ham3tc
        (c, 0.690) +- (0, 0.006)      % mod5d1
        (d, 2.101) +- (0, 0.213)      % gf2\^{}3mult\_11\_47
        (e, 7.010) +- (0, 0.217)      % 4b15g\_1
        (f, 108.961) +- (0, 18.739)   % gf2\^{}4mult\_19\_83
        (g, 890.704) +- (0, 177.617)	% 5mod5tc
        (h, 1258.402) +- (0, 216.143)	% gf2\^{}5mult\_29\_129
        (i, 160.033) +- (0, 94.802)	  % ham7tc
        (j, 1487.176) +- (0, 149.927)	% 5bitadder
    };

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit
    ] coordinates {
        % nocore
                                      % all 0 seed?
        % (a, 0.006) +- (0, 0.002)	    % rd32
        (b, 0.025) +- (0, 0.001)	    % ham3tc
        (c, 0.752) +- (0, 0.018)	    % mod5d1
        (d, 2.160) +- (0, 0.144)	    % gf2\^{}3mult\_11\_47
        (e, 10.206) +- (0, 1.977)	    % 4b15g\_1
        (f, 101.118) +- (0, 12.279)	  % gf2\^{}4mult\_19\_83
        (g, 1578.834) +- (0, 121.287)	% 5mod5tc
        (h, 1284.055) +- (0, 351.351)	% gf2\^{}5mult\_29\_129
        (i, 165.732) +- (0, 98.251)	  % ham7tc
        (j, 902.333) +- (0, 0.000)	% 5bitadder (1 sample)
    };

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit,
    ] coordinates {
        % core naive
    	(b, 0.022) +- (0, 0.000)      % ham3tc
    	(c, 1.247) +- (0, 0.016)      % mod5d1
    	(d, 2.568) +- (0, 0.030)      % gf2\^{}3mult\_11\_47
    	(e, 28.395) +- (0, 2.289)     % 4b15g\_1
    	(f, 23.267) +- (0, 7.848)     % gf2\^{}4mult\_19\_83
    	(g, 1576.194) +- (0, 68.088)	% 5mod5tc
    	(h, 974.229) +- (0, 243.754)	% gf2\^{}5mult\_29\_129
    	(i, 571.523) +- (0, 91.298)	  % ham7tc
    	(j, 1669.661) +- (0, 240.941)	% 5bitadder
    };

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit,
    ] coordinates {
        % nocore naive
        % (0, 0.005) +- (0, 0.000)	    % rd32
        (b, 0.025) +- (0, 0.000)	    % ham3tc
        (c, 1.321) +- (0, 0.035)	    % mod5d1
        (d, 2.716) +- (0, 0.390)	    % gf2\^{}3mult\_11\_47
        (e, 37.784) +- (0, 3.808)	    % 4b15g\_1
        (f, 58.676) +- (0, 13.872)	  % gf2\^{}4mult\_19\_83
        (g, 2246.857) +- (0, 76.189)	% 5mod5tc
        (h, 1021.491) +- (0, 157.994)	% gf2\^{}5mult\_29\_129
        (i, 561.574) +- (0, 56.444)	  % ham7tc
        (j, 1470.711) +- (0, 0.000)	    % 5bitadder (1 sample)
    };
\end{vsplotfour}
\caption{ core vs nocore comparison \\
	a = \texttt{rd32},
	b = \texttt{ham3tc},
	c = \texttt{mod5d1},
  d = \texttt{gf2\^{}3mult\_11\_47},
  e = \texttt{4b15g\_1},
  f = \texttt{gf2\^{}4mult\_19\_83},
  g = \texttt{5mod5tc},
  h = \texttt{gf2\^{}5mult\_29\_129},
  i = \texttt{ham7tc},
  j = \texttt{5bitadder},
}
\end{figure}

% % core - sat.core.minimize_partial
% (0, 0.006) +- (0, 0.000)	% rd32
% (1, 0.024) +- (0, 0.000)	% ham3tc
% (2, 0.732) +- (0, 0.000)	% mod5d1
% (3, 2.123) +- (0, 0.000)	% gf2\^{}3mult\_11\_47
% (4, 5.243) +- (0, 0.000)	% 4b15g\_1
% (5, 147.210) +- (0, 0.000)	% gf2\^{}4mult\_19\_83
% (6, 1575.615) +- (0, 0.000)	% 5mod5tc
% (7, 1271.906) +- (0, 0.000)	% gf2\^{}5mult\_29\_129
% (8, 98.185) +- (0, 0.000)	% ham7tc
% (9, 1077.445) +- (0, 0.000)	% 5bitadder

% % control
% (0, 0.005) +- (0, 0.000)	% rd32
% (1, 0.024) +- (0, 0.000)	% ham3tc
% (2, 1.317) +- (0, 0.000)	% mod5d1
% (3, 1.824) +- (0, 0.000)	% gf2\^{}3mult\_11\_47
% (4, 23.010) +- (0, 0.000)	% 4b15g\_1
% (5, 70.481) +- (0, 0.000)	% gf2\^{}4mult\_19\_83
% (6, 1749.374) +- (0, 0.000)	% 5mod5tc
% (7, 817.749) +- (0, 0.000)	% gf2\^{}5mult\_29\_129
% (8, 545.759) +- (0, 0.000)	% ham7tc
% (9, 1320.959) +- (0, 0.000)	% 5bitadder

% using an unsat-core and generalizing it 
% Vs
% using a partially reduced unsat-core (sat.core.minimize_partial) and
% generalizing it
%   Slight but mostly consistent improvement
\begin{figure}
% \centering
\begin{vsplotfour}
{core \cipdr, min-p \cipdr, core naive \cipdr, min-p naive \cipdr}
{
    % a,
    b,
    c,
    d,
    e,
    f,
    g,
    h,
    i,
    j,
}
    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit
    ] coordinates {
        % core
        (b, 0.022) +- (0, 0.000)      % ham3tc
        (c, 0.690) +- (0, 0.006)      % mod5d1
        (d, 2.101) +- (0, 0.213)      % gf2\^{}3mult\_11\_47
        (e, 7.010) +- (0, 0.217)      % 4b15g\_1
        (f, 108.961) +- (0, 18.739)   % gf2\^{}4mult\_19\_83
        (g, 890.704) +- (0, 177.617)	% 5bitadder
        (h, 1258.402) +- (0, 216.143)	% gf2\^{}5mult\_29\_129
        (i, 160.033) +- (0, 94.802)	  % ham7tc
        (j, 1487.176) +- (0, 149.927)	% 5mod5tc
    };

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit
    ] coordinates {
        % partial minimize
        % (0, 0.005) +- (0, 0.000)	% rd32
        (b, 0.025) +- (0, 0.001)	% ham3tc
        (c, 0.732) +- (0, 0.025)	% mod5d1
        (d, 1.954) +- (0, 0.233)	% gf2\^{}3mult\_11\_47
        (e, 7.039) +- (0, 1.131)	% 4b15g\_1
        (f, 96.225) +- (0, 13.023)	% gf2\^{}4mult\_19\_83
        (g, 1420.482) +- (0, 141.559)	% 5mod5tc
        (h, 1228.083) +- (0, 214.496)	% gf2\^{}5mult\_29\_129
        (i, 161.421) +- (0, 81.533)	% ham7tc
        (j, 1085.111) +- (0, 323.574)	% 5bitadder

    };

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit,
    ] coordinates {
        % core naive
    	(b, 0.022) +- (0, 0.000)      % ham3tc
    	(c, 1.247) +- (0, 0.016)      % mod5d1
    	(d, 2.568) +- (0, 0.030)      % gf2\^{}3mult\_11\_47
    	(e, 28.395) +- (0, 2.289)     % 4b15g\_1
    	(f, 23.267) +- (0, 7.848)     % gf2\^{}4mult\_19\_83
    	(g, 1576.194) +- (0, 68.088)	% 5mod5tc
    	(h, 974.229) +- (0, 243.754)	% gf2\^{}5mult\_29\_129
    	(i, 571.523) +- (0, 91.298)	  % ham7tc
    	(j, 1669.661) +- (0, 240.941)	% 5bitadder
    };

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit,
    ] coordinates {
        % partial minimize
        % (0, 0.005) +- (0, 0.000)	% rd32
        (b, 0.025) +- (0, 0.001)	% ham3tc
        (c, 1.253) +- (0, 0.089)	% mod5d1
        (d, 2.290) +- (0, 0.313)	% gf2\^{}3mult\_11\_47
        (e, 28.217) +- (0, 2.556)	% 4b15g\_1
        (f, 57.623) +- (0, 17.352)	% gf2\^{}4mult\_19\_83
        (g, 1705.183) +- (0, 117.067)	% 5mod5tc
        (h, 952.235) +- (0, 319.049)	% gf2\^{}5mult\_29\_129
        (i, 580.080) +- (0, 113.466)	% ham7tc
        (j, 1308.627) +- (0, 205.371)	% 5bitadder
    };
\end{vsplotfour}
\caption{ core vs minimized (partial) core
	a = \texttt{rd32},
	b = \texttt{ham3tc},
	c = \texttt{mod5d1},
  d = \texttt{gf2\^{}3mult\_11\_47},
  e = \texttt{4b15g\_1},
  f = \texttt{gf2\^{}4mult\_19\_83},
  g = \texttt{5mod5tc},
  h = \texttt{gf2\^{}5mult\_29\_129},
  i = \texttt{ham7tc},
  j = \texttt{5bitadder},
}
\end{figure}

\begin{figure}
% \centering
\begin{vsplot}
{skip-blocked min \cipdr, skip-blocked min naive \cipdr}
{
    % a,
    b,
    c,
    d,
    e,
    f,
    g,
    h,
    i,
    j,
}
    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit
    ] coordinates {
        % ipdr
        % (a, 0.005) +- (0, 0.000)	% rd32
        (b, 0.024) +- (0, 0.000)	% ham3tc
        (c, 0.695) +- (0, 0.032)	% mod5d1
        (d, 1.868) +- (0, 0.264)	% gf2\^{}3mult\_11\_47
        (e, 6.858) +- (0, 0.158)	% 4b15g\_1
        (f, 76.304) +- (0, 10.483)	% gf2\^{}4mult\_19\_83
        (g, 605.231) +- (0, 55.001)	% 5mod5tc
        (h, 939.095) +- (0, 174.136)	% gf2\^{}5mult\_29\_129
        (i, 114.335) +- (0, 38.659)	% ham7tc
        (j, 616.365) +- (0, 156.155)	% 5bitadder
    };

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit
    ] coordinates {
        % naive
        % (a, 0.005) +- (0, 0.000)	% rd32
        (b, 0.024) +- (0, 0.000)	% ham3tc
        (c, 1.126) +- (0, 0.099)	% mod5d1
        (d, 1.829) +- (0, 0.202)	% gf2\^{}3mult\_11\_47
        (e, 21.015) +- (0, 1.570)	% 4b15g\_1
        (f, 16.702) +- (0, 3.801)	% gf2\^{}4mult\_19\_83
        (g, 886.633) +- (0, 100.782)	% 5mod5tc
        (h, 646.602) +- (0, 108.967)	% gf2\^{}5mult\_29\_129
        (i, 313.548) +- (0, 44.443)	% ham7tc
        (j, 1230.704) +- (0, 125.915)	% 5bitadder
    };
    \end{vsplot}
\caption{ skip blocked minimized core
	a = \texttt{rd32},
	b = \texttt{ham3tc},
	c = \texttt{mod5d1},
  d = \texttt{gf2\^{}3mult\_11\_47},
  e = \texttt{4b15g\_1},
  f = \texttt{gf2\^{}4mult\_19\_83},
  g = \texttt{5mod5tc},
  h = \texttt{gf2\^{}5mult\_29\_129},
  i = \texttt{ham7tc},
  j = \texttt{5bitadder},
}
\end{figure}



==> sections/experiments/results/old/results-relax.tex <==
% 2023-03-29
\begin{figure}
% \centering
\begin{vsplot}{\cipdr, naive \cipdr}{
    % a,
    b,
    c,
    d,
    e,
    f,
    g,
    h,
    i,
    j,
}
    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit
    ] coordinates {
        % (a, 0.017) +- (0, 0.002)	% rd32
        (b, 0.033) +- (0, 0.000)	% ham3tc
        (c, 0.730) +- (0, 0.027)	% mod5d1
        (d, 1.463) +- (0, 0.100)	% gf2\^{}3mult\_11\_47
        (e, 25.501) +- (0, 0.951)	% 4b15g\_1
        (f, 25.573) +- (0, 1.430)	% gf2\^{}4mult\_19\_83
        (g, 1656.156) +- (0, 127.014)	% 5mod5tc
        (h, 229.042) +- (0, 36.602)	% gf2\^{}5mult\_29\_129
        (i, 421.544) +- (0, 85.080)	% ham7tc
        (j, 576.068) +- (0, 103.805)	% 5bitadder
        };

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit,
    ] coordinates {
        % (a, 0.017) +- (0, 0.002)	% rd32
        (b, 0.033) +- (0, 0.000)	% ham3tc
        (c, 0.730) +- (0, 0.016)	% mod5d1
        (d, 1.542) +- (0, 0.090)	% gf2\^{}3mult\_11\_47
        (e, 23.933) +- (0, 1.062)	% 4b15g\_1
        (f, 25.658) +- (0, 1.030)	% gf2\^{}4mult\_19\_83
        (g, 1688.681) +- (0, 131.668)	% 5mod5tc
        (h, 404.370) +- (0, 165.632)	% gf2\^{}5mult\_29\_129
        (i, 407.512) +- (0, 82.381)	% ham7tc
        (j, 679.463) +- (0, 138.164)	% 5bitadder
    };
\end{vsplot}
\caption{
    core relaxing pebbling
	a = \texttt{rd32},
	b = \texttt{ham3tc},
	c = \texttt{mod5d1},
  d = \texttt{gf2\^{}3mult\_11\_47},
  e = \texttt{4b15g\_1},
  f = \texttt{gf2\^{}4mult\_19\_83},
  g = \texttt{5mod5tc},
  h = \texttt{gf2\^{}5mult\_29\_129},
  i = \texttt{ham7tc},
  j = \texttt{5bitadder},
} \label{experiments:pebbling:results-relax}
\end{figure}




==> sections/experiments/results/relax/5bitadder-results.tex <==
\begin{figure}[ht]
\centering
\begin{tabular}
{|r|rr|r|}
\hline
 & \ripdr & Naive \ripdr & Improvement \\\hline
avg time & 541.236 s & 775.942 s & 30.25 \% \\
std dev time & 73.874 s & 171.879 s &  \\
max inv constraint & 8 & 8 &  \\
% min inv level & 9 & 8 & 0.00 \% \\
min strat marked & 9 & 9 &  \\
min strat length & 37 & 39 & 5.13 \% \\\hline
\end{tabular}

% CTI graph
\begin{tikzpicture}
    \begin{axis}
    [
%        ymode=log,
%        log origin=infty,
		ymin=0,
        xtick=data,
        xtick style={draw=none},
        minor tick num=1,
        width=\textwidth,
        height=6cm,
        enlarge x limits=0.1,
        enlarge y limits={upper=0},
        xlabel={Maximum Number of Pebbles},
        ybar,
        axis y line*=left,
        bar width=7pt,
        legend style={at={(0.5,1.16)}, anchor=north,legend columns=-1},
        fill between/on layer={main},
    ]
    \legend{cti-count, naive cti-count}

    \errorbarplot{blue}{5bitadder cti-count.dat};

    \errorbarplot{red}{5bitadder naive cti-count.dat};

    \end{axis}
    \begin{axis}
    [
        ymode=log,
        log origin=infty,
        xtick=data,
        xtick style={draw=none},
        minor tick num=1,
        width=\textwidth,
        height=6cm,
        enlarge x limits=0.1,
        enlarge y limits={upper=0},
        axis y line*=right,
        legend style={at={(0.5,1.03)}, anchor=north,legend columns=-1},
        xticklabels={,,},
        ylabel={Time (s)},
        fill between/on layer={main},
    ]
    \legend{cti-time, naive cti-time}

    \dotplot{blue}{5bitadder cti-time.dat};
    \addplot [name path=upper,draw=none]
        table[x=x,y expr=\thisrow{y}+\thisrow{err}] {5bitadder cti-time.dat};
    \addplot [name path=lower,draw=none] 
        table[x=x,y expr=\thisrow{y}-\thisrow{err}] {5bitadder cti-time.dat};
    \filldevplot{blue}

    \dotplot{red}{5bitadder naive cti-time.dat};
    \addplot [name path=upper,draw=none]
        table[x=x,y expr=\thisrow{y}+\thisrow{err}] {5bitadder naive cti-time.dat};
    \addplot [name path=lower,draw=none] 
        table[x=x,y expr=\thisrow{y}-\thisrow{err}] {5bitadder naive cti-time.dat};
    \linedevplot{red}

    \end{axis}
    \end{tikzpicture}
    \caption{
        Statistics for the relaxing \texttt{5bitadder} experiment, averaged over each
        repetition. This graph compares the number of counterexamples (cti-count)
        on the left axis found in the major iteration and the total runtime
        (cti-time) on the right axis of the algorithm.
    }
	\label{fig:pebbling:relax:5bit:cti}
\end{figure}

{
% \newlength{\plotheight}
% \setlength{9cm}
\newcommand{\plotheight}{6cm}
% Obligation graph
\begin{figure}[ht]
    \centering
    \begin{subfigure}{\textwidth}
    \begin{tikzpicture}
    \begin{axis}
    [
%        ymode=log,
%        log origin=infty,
		ymin=0,
        xtick=data,
        xtick style={draw=none},
        minor tick num=1,
        height=\plotheight,
        width=\textwidth,
        enlarge x limits=0.1,
        enlarge y limits={upper=0},
        xlabel={Maximum Number of Pebbles},
        ybar,
        axis y line*=left,
        bar width=7pt,
        legend style={at={(0.5,1.13)}, anchor=north,legend columns=-1},
        ylabel={No. obligations},
        fill between/on layer={main},
    ]
    \legend{obligation-count, naive obligation-count}

    \errorbarplot{blue}{5bitadder obligation-count.dat};

    \errorbarplot{red}{5bitadder naive obligation-count.dat};

    \end{axis}
    \begin{axis}
    [
        ymode=log,
        log origin=infty,
        xtick=data,
        xtick style={draw=none},
        minor tick num=1,
        height=\plotheight,
        width=\textwidth,
        enlarge x limits=0.1,
        enlarge y limits={upper=0},
        axis y line*=right,
        legend style={at={(0.5,1.0)}, anchor=north,legend columns=-1},
        xticklabels={,,},
        ylabel={Time (s)},
        fill between/on layer={main},
    ]
    \legend{obligation-time, naive obligation-time}

    \dotplot{blue}{5bitadder obligation-time.dat}
    \addplot [name path=upper,draw=none]
        table[x=x,y expr=\thisrow{y}+\thisrow{err}] {5bitadder obligation-time.dat};
    \addplot [name path=lower,draw=none] 
        table[x=x,y expr=\thisrow{y}-\thisrow{err}] {5bitadder obligation-time.dat};
    \filldevplot{blue}

    \dotplot{red}{5bitadder naive obligation-time.dat};
    \addplot [name path=upper,draw=none]
        table[x=x,y expr=\thisrow{y}+\thisrow{err}] {5bitadder naive obligation-time.dat};
    \addplot [name path=lower,draw=none] 
        table[x=x,y expr=\thisrow{y}-\thisrow{err}] {5bitadder naive obligation-time.dat};
    \linedevplot{red}

    \end{axis}

    \end{tikzpicture}
    \caption{
        This graph compares the total number of obligations (obligation-count)
        handled by the minor iteration on the left axis and the time spent on
        them (obligation-time) on the right axis.
    }
	\label{fig:pebbling:relax:5bit:obl}
    \end{subfigure}

    \begin{subfigure}{\textwidth}
    % SAT-call graph
    \begin{tikzpicture}
    \begin{axis}
    [
%        ymode=log,
%        log origin=infty,
		ymin=0,
        xtick=data,
        xtick style={draw=none},
        minor tick num=1,
        height=\plotheight,
        width=\textwidth,
        enlarge x limits=0.1,
        enlarge y limits={upper=0},
        xlabel={Maximum Number of Pebbles},
        ybar,
        axis y line*=left,
        bar width=7pt,
        legend style={at={(0.5,1.13)}, anchor=north,legend columns=-1},
        ylabel={No. \sat-queries},
        fill between/on layer={main},
    ]
    \legend{sat-count, naive sat-count}

    \errorbarplot{blue}{5bitadder sat-count.dat};

    \errorbarplot{red}{5bitadder naive sat-count.dat};

    \end{axis}
    \begin{axis}
    [
        ymode=log,
        log origin=infty,
        xtick=data,
        xtick style={draw=none},
        minor tick num=1,
        height=\plotheight,
        width=\textwidth,
        enlarge x limits=0.1,
        enlarge y limits={upper=0},
        axis y line*=right,
        legend style={at={(0.5,1.0)}, anchor=north,legend columns=-1},
        xticklabels={,,},
        ylabel={Time (s)},
        fill between/on layer={main},
    ]
    \legend{sat-time, naive sat-time}

    \dotplot{blue}{5bitadder sat-time.dat}
    \addplot [name path=upper,draw=none]
        table[x=x,y expr=\thisrow{y}+\thisrow{err}] {5bitadder sat-time.dat};
    \addplot [name path=lower,draw=none] 
        table[x=x,y expr=\thisrow{y}-\thisrow{err}] {5bitadder sat-time.dat};
    \filldevplot{blue}

    \dotplot{red}{5bitadder naive sat-time.dat}
    \addplot [name path=upper,draw=none]
        table[x=x,y expr=\thisrow{y}+\thisrow{err}] {5bitadder naive sat-time.dat};
    \addplot [name path=lower,draw=none] 
        table[x=x,y expr=\thisrow{y}-\thisrow{err}] {5bitadder naive sat-time.dat};
    \linedevplot{red}

    \end{axis}
    \end{tikzpicture}
    \caption{
        The total number of calls to the \sat-solver (sat-count) on the left
        axis and the total time spent waiting on the \sat-solver (sat-time) on
        the right.
    }
	\label{fig:pebbling:relax:5bit:sat}
    \end{subfigure}
    \caption{Statistics for the relaxing \texttt{5bitadder} experiment, averaged over each repetition.}
    \label{fig:pebbling:relax:5bit:oblsat}
\end{figure}
}

% Frames after relaxing
{
\newcommand{\plotheight}{5cm}
\begin{figure}[ht]
    \vspace*{-2cm}
    \begin{subfigure}{\textwidth}
    \begin{tikzpicture}
    \begin{axis}
    [
        xtick=data,
        xtick style={draw=none},
        minor tick num=1,
        height=\plotheight,
        width=\textwidth,
        enlarge x limits=0.1,
        enlarge y limits={upper=0},
        xlabel={Frames per Constraint},
        ybar=1pt,
        axis y line*=left,
        bar width=0pt,
        legend style={at={(0.3,1.16)}, anchor=north,legend columns=-1},
        ylabel={No. cubes},
    ]
    \legend{relax-frames-pre}

    \addplot [draw=black, fill=black]
        table [x=x, y=f1, y error=f1err] {5bitadder relax-frames-pre.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f2, y error=f2err] {5bitadder relax-frames-pre.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f3, y error=f3err] {5bitadder relax-frames-pre.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f4, y error=f4err] {5bitadder relax-frames-pre.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f5, y error=f5err] {5bitadder relax-frames-pre.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f6, y error=f6err] {5bitadder relax-frames-pre.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f7, y error=f7err] {5bitadder relax-frames-pre.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f8, y error=f8err] {5bitadder relax-frames-pre.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f9, y error=f9err] {5bitadder relax-frames-pre.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f10, y error=f10err] {5bitadder relax-frames-pre.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f11, y error=f11err] {5bitadder relax-frames-pre.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f12, y error=f12err] {5bitadder relax-frames-pre.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f13, y error=f13err] {5bitadder relax-frames-pre.dat};

    \end{axis}

    \begin{axis}
    [
        xtick=data,
        xtick style={draw=none},
        minor tick num=1,
        height=\plotheight,
        width=\textwidth,
        enlarge x limits=0.1,
        enlarge y limits={upper=0},
        axis y line*=right,
        legend style={at={(0.7,1.16)}, anchor=north,legend columns=-1},
        xticklabels={,,},
        ylabel={Copyrate (\%)},
    ]
    \legend{relax-frames-perc}

    \addplot+[blue,mark=x, mark size=4pt, x=x, y=y] table {5bitadder relax-frames-perc.dat};
    \addplot [name path=upper,draw=none]
        table[x=x,y expr=\thisrow{y}+\thisrow{err}] {5bitadder relax-frames-perc.dat};
    \addplot [name path=lower,draw=none] 
        table[x=x,y expr=\thisrow{y}-\thisrow{err}] {5bitadder relax-frames-perc.dat};
    \addplot [fill=blue!20] fill between[of=upper and lower];
    \end{axis}

    \end{tikzpicture}
    \caption{
        The amount of cubes learned at the end of the individual \pdr run, but
        before copying them to the next instance, (relax-frames-pre) for each
        constraint. The line shows the percentage of cube-levels that could be
        carried over to the next instance.
    }
    \end{subfigure}

    \begin{subfigure}{\textwidth}
    \begin{tikzpicture}
    \begin{axis}
    [
        xtick=data,
        xtick style={draw=none},
        minor tick num=1,
        height=\plotheight,
        width=\textwidth,
        enlarge x limits=0.1,
        enlarge y limits={upper=0},
        xlabel={Frames per Constraint},
        ybar=1pt,
        axis y line*=left,
        bar width=0pt,
        legend style={at={(0.3,1.16)}, anchor=north,legend columns=-1},
        ylabel={No. cubes},
    ]
    \legend{relax-frames-post}

    \addplot [draw=black, fill=black]
        table [x=x, y=f1, y error=f1err] {5bitadder relax-frames-post.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f2, y error=f2err] {5bitadder relax-frames-post.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f3, y error=f3err] {5bitadder relax-frames-post.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f4, y error=f4err] {5bitadder relax-frames-post.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f5, y error=f5err] {5bitadder relax-frames-post.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f6, y error=f6err] {5bitadder relax-frames-post.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f7, y error=f7err] {5bitadder relax-frames-post.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f8, y error=f8err] {5bitadder relax-frames-post.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f9, y error=f9err] {5bitadder relax-frames-post.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f10, y error=f10err] {5bitadder relax-frames-post.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f11, y error=f11err] {5bitadder relax-frames-post.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f12, y error=f12err] {5bitadder relax-frames-post.dat};
    \addplot [draw=black, fill=black]
        table [x=x, y=f13, y error=f13err] {5bitadder relax-frames-post.dat};

    \end{axis}

    \begin{axis}
    [
        xtick=data,
        xtick style={draw=none},
        minor tick num=1,
        height=\plotheight,
        width=\textwidth,
        enlarge x limits=0.1,
        enlarge y limits={upper=0},
        axis y line*=right,
        legend style={at={(0.7,1.16)}, anchor=north,legend columns=-1},
        xticklabels={,,},
        ylabel={Copyrate (\%)},
    ]
    \legend{relax-frames-perc}

    \addplot+[blue,mark=x, mark size=4pt, x=x, y=y] table {5bitadder relax-frames-perc.dat};
    \addplot [name path=upper,draw=none]
        table[x=x,y expr=\thisrow{y}+\thisrow{err}] {5bitadder relax-frames-perc.dat};
    \addplot [name path=lower,draw=none] 
        table[x=x,y expr=\thisrow{y}-\thisrow{err}] {5bitadder relax-frames-perc.dat};
    \addplot [fill=blue!20] fill between[of=upper and lower];
    \end{axis}
    \end{tikzpicture}
    \caption{
        The amount of cubes that could be carried over the next instance
        (relax-frames-post) and the same carry-over percentage
        (relax-frames-prec).
    }
    \end{subfigure}
    \caption{
        Statistics for the carry-over of cubes between relaxing instances for
        the \texttt{5bitadder} relaxing experiment, averaged over each repetition. For
        each constraint, the bargraph shows cubes learned at each level in the
        delta-encoding.
    } \label{fig:pebbling:relax:5bit:copy}
\end{figure}
}


==> sections/experiments/results/relax/5mod5tc.tex <==
\begin{figure}[ht]
	\centering
	\begin{tabular}
		{|r|rr|r|}
		\hline
		& \ripdr & Naive \ripdr & Improvement \\\hline
		avg time & 747.978 s & 845.274 s & 11.51 \% \\
		std dev time & 106.465 s & 80.059 s &  \\
		avg incremental time & 0.455 s &  &  \\
		std dev incremental time & 0.009 s &  &  \\
		max inv constraint & 5 & 5 &  \\
%		min inv level & 9 & 5 & 0.00 \% \\
		min strat marked & 6 & 6 &  \\
		min strat length & 37 & 41 & 9.76 \% \\\hline
	\end{tabular}
	
\begin{subfigure}{\textwidth}
	% CTI graph
	\begin{tikzpicture}
	    \begin{axis}
     [
	%        ymode=log,
	%        log origin=infty,
	        xtick=data,
	        xtick style={draw=none},
	        x axis line style={draw=none},
	        minor tick num=1,
	        height=6cm,
	        width=\textwidth,
	        enlarge x limits=0.05,
	        enlarge y limits={upper=0},
	        xlabel={Maximum Number of Pebbles},
	        ybar,
	        axis y line*=left,
	        bar width=7pt,
	        legend style={at={(0.5,1.17)}, anchor=north,legend columns=-1},
	        ylabel={No. ctis},
	        fill between/on layer={main},
     ]
	        \legend{\ripdr cti-count, naive cti-count}

					\pgfplotstableread{
            x y err
            1 0 0
            2 1 0
            3 8 0
            4 1 0
            5 2 0
            6 6.2 3.283900120283807
	        }\cticount
	        \errorbarplot{blue}{\cticount};

					\pgfplotstableread{
            x y err
            1 0 0
            2 1 0
            3 9 0
            4 9 0
            5 9 0
            6 9 0
	        }\ncticount
	        \errorbarplot{red}{\ncticount};
			\end{axis}

	    \begin{axis}
			[
	        ymode=log,
	        log origin=infty,
	        xtick=data,
	        xtick style={draw=none},
	        minor tick num=1,
	        height=6cm,
	        width=\textwidth,
	        enlarge x limits=0.05,
	        enlarge y limits={upper=0},
	        axis y line*=right,
	        legend style={at={(0.5,1.05)}, anchor=north,legend columns=-1},
	        xticklabels={,,},
	        ylabel={Time (s)},
	        fill between/on layer={main},
			]
	        \legend{\ripdr cti-time, naive cti-time}

					\pgfplotstableread{
            x y err
            1 0.0012483292 1.6836555032428678e-05
            2 0.0263717689 0.0011561732692866112
            3 2.2954469898000003 0.015698926077071677
            4 6.7017508957 0.155353896682409
            5 613.9713969267001 31.610254247090182
            6 124.52625216290001 93.6093225466821
	        }\ctitime
	        \dotplot{blue}{\ctitime};
	        \addplot [name path=upper,draw=none]
						table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\ctitime};
	        \addplot [name path=lower,draw=none] 
						table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\ctitime};
	        \filldevplot{blue}

					\pgfplotstableread{
            x y err
            1 0.0012424737 2.2005527214997587e-05
            2 0.0237144431 0.0015518347855024033
            3 2.3310425605 0.04255697723874949
            4 10.8031158487 0.4392294294950168
            5 756.1265161801001 87.0623408821032
            6 75.68233309950001 34.31181456971805
	        }\nctitime
	        \dotplot{red}{\nctitime};
	        \addplot [name path=upper,draw=none]
	        	table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\nctitime};
	        \addplot [name path=lower,draw=none] 
	        	table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\nctitime};
	        \linedevplot{red}
	        
	    \end{axis}
	    %\caption{Statistics for 5mod5tc experiment.}
	    
	\end{tikzpicture}
	\caption{
		A comparison between the number of counterexamples found in the major
		iteration (cti-count) on the left axis and the total runtime (cti-time)
		on the right axis.
	}
	\label{fig:pebbling:relax:5mod5tc:cti}
	\end{subfigure}
	
	\begin{subfigure}{\textwidth}
		\centering
	% Incremental times
	\begin{tikzpicture}		
		\begin{axis}
			[
				ymin=0,
				xtick=data,
				xtick style={draw=none},
				minor tick num=1,
				height=4cm,
				width=0.8\textwidth,
				enlarge x limits=0.1,
				enlarge y limits={upper=0},
				ybar,
				axis y line*=right,
				xticklabels={,,},
				bar width=7pt,
				legend style={at={(0.52,1.38)}, anchor=north,legend columns=-1},
				ylabel={Copyrate (\%)},
				fill between/on layer={main},
			]
			\legend{\ipdr copyrate}

			\pgfplotstableread{
        x y err
        2 0 0
        3 50 0
        4 84.79999999999998 1.4210854715202004e-14
        5 53.09278350515466 1.4210854715202004e-14
        6 28.76372779723032 0.9673007781174193
			}\incperc
			\errorbarplot{blue}{\incperc};
		\end{axis}
	
		\begin{axis}
		[
			xtick=data,
			xtick style={draw=none},
			minor tick num=1,
			height=4cm,
			width=0.8\textwidth,
			enlarge x limits=0.05,
			enlarge y limits={upper=0},
			xlabel={Maximum Number of Pebbles},
			axis y line*=left,
			legend style={at={(0.52,1.16)}, anchor=north,legend columns=-1},
			ylabel={Time (s)},
			fill between/on layer={main},
		]
			\legend{\ripdr inc-time, naive inc-time}

			\pgfplotstableread{
        x y err
        2 0.0021967583 0.00020658864409064208
        3 0.0033233758 0.0002901697160979416
        4 0.060769884399999995 0.0002409681175405563
        5 0.059251724900000004 0.00027286923564867133
        6 0.3299074019 0.008687649287945928
			}\inctime
			\dotplot{blue}{\inctime};
			\addplot [name path=upper,draw=none]
				table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\inctime};
			\addplot [name path=lower,draw=none] 
				table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\inctime};
			\filldevplot{blue}

			\pgfplotstableread{
  	     x y err
         2 0.06372667409999999 0.0015392018508383132
         3 0.058139477800000006 0.0019239595589074516
         4 0.05680836609999999 0.00018198586632178388
         5 0.0576721806 9.792532550591828e-05
         6 0.0700625295 0.0007930261586262126
			}\ninctime
		\dotplot{red}{\ninctime};
		\addplot [name path=upper,draw=none]
			table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\ninctime};
		\addplot [name path=lower,draw=none] 
			table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\ninctime};
		\linedevplot{red}
		\end{axis}
	\end{tikzpicture}
	\caption{
		The amount of the runtime that was spent on copying clauses to the
		relaxed instance denoted on the x-axis. This number is already included
		in the times of the upper graph. 
	}
	\label{relax}
	\end{subfigure}

    \caption{
	    Statistics for the relaxing \texttt{5mod5tc} experiment,
	    averaged over 10 repetitions.
    }\label{fig:pebbling:relax:5mod5tc}
\end{figure}

{
\newcommand{\plotheight}{6cm}
% Obligation graph
	\begin{figure}[h]
	\centering
	\begin{subfigure}{\textwidth}
	\begin{tikzpicture}
	    \begin{axis}
			[
				 ymode=log,
				 log origin=infty,
				xtick=data,
				xtick style={draw=none},
				minor tick num=1,
				height=\plotheight,
				width=\textwidth,
				enlarge x limits=0.05,,
				enlarge y limits={upper=0},
				xlabel={Maximum Number of Pebbles},
				ybar,
				axis y line*=left,
				bar width=7pt,
				legend style={at={(0.5,1.19)}, anchor=north,legend columns=-1},
				ylabel={No. obligations},
				fill between/on layer={main},
			]		
	        \legend{\ripdr obligation-count, naive obligation-count}

	        \pgfplotstableread{
            x y err
            1 1 0
            2 1 0
            3 20 0
            4 31 0
            5 524.3 13.96026504046395
            6 419.2 173.35283095467463
	        }\oblcount
        	\errorbarplot{blue}{\oblcount};

					\pgfplotstableread{
            x y err
            1 1 0
            2 1 0
            3 22 0
            4 49.9 0.03162277660168424
            5 583.4 36.07957871150936
            6 369.1 81.85597717943388
	        }\noblcount
        	\errorbarplot{red}{\noblcount};
      	\end{axis}

	    \begin{axis}
        [
          ymode=log,
          log origin=infty,
					xtick=data,
					xtick style={draw=none},
					minor tick num=1,
					height=\plotheight,
					width=\textwidth,
					enlarge x limits=0.05,,
					enlarge y limits={upper=0},
					axis y line*=right,
					legend style={at={(0.5,1.06)}, anchor=north,legend columns=-1},
					xticklabels={,,},
					ylabel={Time (s)},
					fill between/on layer={main},
				]
	        \legend{\ripdr obligation-time, naive obligation-time}

					\pgfplotstableread{
            x y err
            1 0.0012483292 1.6836555032428678e-05
            2 0.024738739000000003 0.0011635190292320107
            3 2.1884793233 0.014223917173197164
            4 6.5550439899 0.15260534357933647
            5 612.0168259710001 31.578913301551747
            6 123.9301723756 93.22485624129506
	        }\obltime
	        \dotplot{blue}{\obltime};
					\addplot [name path=upper,draw=none]
						table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\obltime};
					\addplot [name path=lower,draw=none] 
						table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\obltime};
					\filldevplot{blue}

					\pgfplotstableread{
            x y err
            1 0.0012424737 2.2005527214997587e-05
            2 0.022030913 0.0015352626014402875
            3 2.2118936142 0.03996876534202263
            4 10.6392157193 0.43008858235922254
            5 753.8600877243 86.94582677319737
            6 75.4847941922 34.30786797661093
	        }\nobltime
        \dotplot{red}{\nobltime};
	    \addplot [name path=upper,draw=none]
			table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\nobltime};
		\addplot [name path=lower,draw=none] 
			table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\nobltime};
		\linedevplot{red}
	    \end{axis}
	    %\caption{Statistics for 5mod5tc experiment.}
	    
	\end{tikzpicture}
	\caption{
	    Left axis: total number of obligations (obligation-count)
	    handled by the minor iteration. Right axis: the time spent on
	    them (obligation-time). For constraint 1, no obligations were enqueued as \pdr terminated in the initialization step. Its obligation-count value was set to 1 to accommodate the logarithmic scale and the obligation-time to the total runtime (which is a close approximation).
	}\label{fig:pebbling:relax:5mod5tc:obl}
	\end{subfigure}
	
	\begin{subfigure}{\textwidth}
	% SAT-call graph
	\begin{tikzpicture}
	    \begin{axis}
        [
					ymode=log,
					log origin=infty,
					xtick=data,
					xtick style={draw=none},
					minor tick num=1,
					height=\plotheight,
					width=\textwidth,
					enlarge x limits=0.05,,
					enlarge y limits={upper=0},
					xlabel={Maximum Number of Pebbles},
					ybar,
					axis y line*=left,
					bar width=7pt,
					legend style={at={(0.5,1.18)}, anchor=north,legend columns=-1},
					ylabel={No. \sat-queries},
					fill between/on layer={main},
				]
	        \legend{\ripdr sat-count, naive sat-count}

        	\pgfplotstableread{
            x y err
            1 2 0
            2 19 0
            3 1252.8 0.7509993342207386
            4 2356.9 13.495962359165034
            5 43875.9 961.366444702539
            6 20973.2 9945.514804372873
	        }\satcount
        	\errorbarplot{blue}{\satcount}

					\pgfplotstableread{
            x y err
            1 2 0
            2 19.5 0.11180339887498948
            3 1279.35 26.56861164983975
            4 3167.3 812.4085760871804
            5 45989.05 3143.770238920936
            6 18577.35 8066.646725320566
					}\nsatcount
					\errorbarplot{red}{\nsatcount}
			\end{axis}
	
	    \begin{axis}
		[
			ymode=log,
			log origin=infty,
			xtick=data,
			xtick style={draw=none},
			minor tick num=1,
			height=\plotheight,
			width=\textwidth,
			enlarge x limits=0.05,,
			enlarge y limits={upper=0},
			axis y line*=right,
			legend style={at={(0.5,1.05)}, anchor=north,legend columns=-1},
			xticklabels={,,},
			ylabel={Time (s)},
			fill between/on layer={main},
		]
	        \legend{\ripdr sat-time, naive sat-time}

        	\pgfplotstableread{
            x y err
            1 0.0003175556 5.660233267277935e-06
            2 0.019026848000000002 0.0012534974469358125
            3 1.1633065488999998 0.013967435356438386
            4 4.304545867199999 0.14556473897765435
            5 549.4729291080992 29.939342477003805
            6 99.77487534890005 80.32393545617971
	        }\sattime
	        \dotplot{blue}{\sattime};
					\addplot [name path=upper,draw=none]
						table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\sattime};
					\addplot [name path=lower,draw=none] 
						table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\sattime};
					\filldevplot{blue}

					\pgfplotstableread{
            x y err
            1 0.000316727 4.198183118921794e-06
            2 0.01811479355 0.0016118688068850228
            3 1.1692165388499998 0.028701536691250085
            4 5.403966850499996 1.1345368777137628
            5 616.1113416441497 90.5592300454616
            6 78.26285115530001 64.01163331418134
	        }\nsattime
        \dotplot{red}{\nsattime};
				\addplot [name path=upper,draw=none]
					table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\nsattime};
				\addplot [name path=lower,draw=none] 
					table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\nsattime};
				\linedevplot{red}
	    \end{axis}
	\end{tikzpicture}
	\caption{
			Left axis: the total number of calls to the \sat-solver (sat-count).
			Right axis: the total time spent waiting on the \sat-solver (sat-time).
	}\label{fig:pebbling:relax:5mod5tc:sat}
	\end{subfigure}
	\caption{
		Relaxing \texttt{5mod5tc} experiment (10 repetitions). Left axis: the number
		of counterexamples (cti-count) found in the major iteration. Right axis:
		the total runtime (cti-time).
	}
	\label{fig:pebbling:relax:5mod5tc:oblsat}
	\end{figure}
}

==> sections/experiments/results/relax/simple.tex <==
\begin{figure}
\begin{center}
\begin{tabular}{|ll|rr|r|}
    \hline
    & Name                           & \ripdr & Naive \ripdr & Improvement \\\hline
    b & \texttt{ham3tc}                & \\
    c & \texttt{mod5d1}                &\\ 
	d & \texttt{gf2\^{}3mult\_11\_47}  &\\
    e & \texttt{4b15g\_1}              &\\
    f & \texttt{gf2\^{}4mult\_19\_83}  &\\
    g & \texttt{5mod5tc}               &\\
    h & \texttt{gf2\^{}5mult\_29\_129} &\\
    i & \texttt{ham7tc}                &\\
    j & \texttt{5bitadder}             &\\
\end{tabular}
\end{center}

% \centering
\begin{vsplot}{constrained copy, simple copy}{
    a,
    b,
    c,
    d,
    e,
    f,
    g,
    h,
    i,
    j,
}
    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit,
    ] coordinates {
        % (a, 0.056) +- (0, 0.005)	% rd32
        (b, 0.044) +- (0, 0.001)	% ham3tc
        (c, 1.126) +- (0, 0.009)	% mod5d1
        (d, 1.999) +- (0, 0.156)	% gf2\^{}3mult\_11\_47
        (e, 31.045) +- (0, 0.358)	% 4b15g\_1
        (f, 9.341) +- (0, 0.556)	% gf2\^{}4mult\_19\_83
        (g, 917.887) +- (0, 75.688)	% 5mod5tc
        (h, 336.332) +- (0, 24.446)	% gf2\^{}5mult\_29\_129
        (i, 280.281) +- (0, 92.384)	% ham7tc
        (j, 683.014) +- (0, 159.848)	% 5bitadder
			% (a, 0.061) +- (0, 0.006)	% rd32
			% (b, 0.047) +- (0, 0.002)	% ham3tc
			% (c, 1.138) +- (0, 0.017)	% mod5d1
			% (d, 1.941) +- (0, 0.157)	% gf2\^{}3mult\_11\_47
			% (e, 31.136) +- (0, 0.343)	% 4b15g\_1
			% (f, 8.994) +- (0, 0.277)	% gf2\^{}4mult\_19\_83
			% (g, 878.740) +- (0, 100.217)	% 5mod5tc
			% (h, 327.893) +- (0, 35.227)	% gf2\^{}5mult\_29\_129
			% (i, 354.319) +- (0, 141.578)	% ham7tc
			% (j, 639.828) +- (0, 216.228)	% 5bitadder    
		};

    \addplot+[
        error bars/.cd,
        y dir=both,
        y explicit
    ] coordinates {
			% (a, 0.026) +- (0, 0.000)	% rd32
			(b, 0.045) +- (0, 0.001)	% ham3tc
			(c, 0.902) +- (0, 0.039)	% mod5d1
			(d, 1.670) +- (0, 0.113)	% gf2\^{}3mult\_11\_47
			(e, 27.114) +- (0, 1.866)	% 4b15g\_1
			(f, 8.303) +- (0, 0.278)	% gf2\^{}4mult\_19\_83
			(g, 903.888) +- (0, 97.502)	% 5mod5tc
			(h, 344.001) +- (0, 15.794)	% gf2\^{}5mult\_29\_129
			(i, 197.956) +- (0, 38.787)	% ham7tc
			(j, 655.619) +- (0, 169.967)	% 5bitadder    
		};

\end{vsplot}
\caption{
Experimental results for the relaxing \ipdr (\ripdr) from
\autoref{ipdr:relaxing}, using the Reversible Pebbling Game from
\autoref{imp:pebbling}. This compares the runtimes from the Constrained Copy
tactic from \autoref{ipdr:relax:constrained-cubes} against the regular copying
method from \autoref{ipdr:relaxing}.
}
 \label{fig:pebbling:relax:all}
\end{figure}




==> sections/experiments/results/stat-figures/4proc-relax.tex <==
{
\newcommand{\plotheight}{6cm}
% Obligation graph
\begin{figure}[ht]
\centering
\begin{subfigure}{\textwidth}
\begin{tikzpicture}
\begin{axis}
	[
	ymode=log,
	log origin=infty,
	xtick=data,
	xtick style={draw=none},
	minor tick num=1,
	height=\plotheight,
	width=\textwidth,
	enlarge x limits=0.05,,
	enlarge y limits={upper=0},
	xlabel={Maximum Number of context switches},
	ybar,
	axis y line*=left,
	bar width=7pt,
	legend style={at={(0.5,1.17)}, anchor=north,legend columns=-1},
	ylabel={No. obligations},
	fill between/on layer={main},
	]		
	\legend{\ripdr obligation-count, naive obligation-count}
	%	        \begin{filecontents}{ham7tc obligation-count.dat}
		\pgfplotstableread{
			x y err
    0 276.6666666666667 91.08258360980456
			1 578 133.09645625134678
			2 1698 277.6040345528141
			3 1772 280.871263511714
		}\oblcount
		\errorbarplot{blue}{\oblcount};
		%	        \begin{filecontents}{ham7tc naive obligation-count.dat}
			\pgfplotstableread{
				x y err
		    0 276.6666666666667 91.08258360980456
				1 629 89.54328562209453
				2 1553.6666666666667 190.5702942145943
				3 3936 128.90565025113006
			}\noblcount
			\errorbarplot{red}{\noblcount};
\end{axis}

\begin{axis}
	[
	ymode=log,
	log origin=infty,
	xtick=data,
	xtick style={draw=none},
	minor tick num=1,
	height=\plotheight,
	width=\textwidth,
	enlarge x limits=0.05,,
	enlarge y limits={upper=0},
	axis y line*=right,
	legend style={at={(0.5,1.04)}, anchor=north,legend columns=-1},
	xticklabels={,,},
	ylabel={Time (s)},
	fill between/on layer={main},
	]
	\legend{\ripdr obligation-time, naive obligation-time}
	%	        \begin{filecontents}{ham7tc obligation-time.dat}
		\pgfplotstableread{
			x y err
	    0 30.904991565 8.40386617189863
			1 261.71103614066664 65.19025482113047
			2 2211.555925235 620.814298109431
			3 2999.8427126716674 867.1718609971315
		}\obltime
		\dotplot{blue}{\obltime};
		\addplot [name path=upper,draw=none]
		table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\obltime};
		\addplot [name path=lower,draw=none] 
		table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\obltime};
		\filldevplot{blue}
		%	        \begin{filecontents}{ham7tc naive obligation-time.dat}
			\pgfplotstableread{
				x y err
		    0 31.000653090999993 8.401838004882366
				1 241.47052277166662 36.21597796421707
				2 1223.3217029119996 248.8063503849408
				3 7985.181220806674 932.7863237848143
			}\nobltime
			\dotplot{red}{\nobltime};
			\addplot [name path=upper,draw=none]
			table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\nobltime};
			\addplot [name path=lower,draw=none] 
			table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\nobltime};
			\linedevplot{red}
\end{axis}
%\caption{Statistics for 4procs experiment.}

\end{tikzpicture}

\caption{
    This graph compares the total number of obligations (obligation-count)
    handled by the minor iteration on the left axis and the time spent on
    them (obligation-time) on the right axis.
}\label{fig:peter:relax:4proc:obl}
\end{subfigure}

    \begin{subfigure}{\textwidth}
    	\centering
    % Incremental times
    \begin{tikzpicture}
				\begin{axis}
			[
				ymin=0,
				xtick=data,
				xtick style={draw=none},
				minor tick num=1,
				height=4cm,
				width=0.8\textwidth,
				enlarge x limits=0.1,
				enlarge y limits={upper=0},
				ybar,
				axis y line*=right,
				xticklabels={,,},
				bar width=7pt,
				legend style={at={(0.52,1.45)}, anchor=north,legend columns=-1},
				ylabel={Copyrate (\%)},
				fill between/on layer={main},
			]
			\legend{\ripdr copyrate}
			% \begin{filecontents}{5bitadder relax-frames-perc (relax).dat}
				\pgfplotstableread{
					x y err
			    1 34.38237952819207 4.507638444841585
					2 43.93369297918042 3.8094062104834636
					3 42.99150156629475 6.951986358854146
				}\incperc
				\errorbarplot{blue}{\incperc};
			\end{axis}
    	
    \begin{axis}
    [
        ymode=log,
				log origin=infty,
        xtick=data,
        xtick style={draw=none},
        minor tick num=1,
        height=4cm,
        width=0.8\textwidth,
        enlarge x limits=0.1,
        enlarge y limits={upper=0},
        xlabel={Maximum number of context switches},
        axis y line*=left,
        legend style={at={(0.5,1.1)}, anchor=north,legend columns=-1},
        ylabel={Time (s)},
    ]
		\legend{\ripdr inc-time, naive inc-time}
		%			\begin{filecontents}{ham7tc inc-time (relax).dat}
			\pgfplotstableread{
				x y err
		    1 1.591105994 0.3820612356361238
				2 9.134560197333332 1.3397921296984834
				3 101.19338122900001 33.42184929164526
			}\inctime
			\dotplot{blue}{\inctime};
			\addplot [name path=upper,draw=none]
			table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\inctime};
			\addplot [name path=lower,draw=none] 
			table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\inctime};
			\filldevplot{blue}
	%			\begin{filecontents}{ham7tc naive inc-time (relax).dat}
			\pgfplotstableread{
				x y err
		    1 0.47466611966666666 0.0009166446212170848
				2 0.486427065 0.0031833461686044525
				3 0.4882934906666667 0.005215346325370431
			}\ninctime
			\dotplot{red}{\ninctime};
			\addplot [name path=upper,draw=none]
			table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\ninctime};
			\addplot [name path=lower,draw=none] 
			table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\ninctime};
			\linedevplot{red}
	    \end{axis}
    \end{tikzpicture}
    \caption{
        The amount of the runtime that was spent on copying clauses to the
        relaxed instance denoted on the x-axis. This number is already included
        in the times of the upper graph. The bars denote the percentage (right y-axis) of clauses that could be copied to the instance with the bound on the x-axis.
    }\label{fig:peter:relax:4proc:inc}
    \end{subfigure}
    \caption{
        Statistics for the relaxing \ttfunction{Peterson}[4] experiment,
        averaged over 3 repetitions.
    }
	\label{fig:peter:relax:4proc}

\end{figure}
}

==> sections/experiments/results/stat-figures/ham7tc-constrain.tex <==
\begin{figure}[h!]
\newcommand{\plotheight}{5cm}
	\centering
%	\begin{subfigure}{\textwidth}
\begin{minipage}{.49\textwidth}
	\begin{tikzpicture}
	    \begin{axis}
		[
        	ymode=log,
			log origin=infty,
			xtick=data,
			xtick style={draw=none},
			x axis line style={draw=none},
			minor tick num=1,
			height=\plotheight,
			width=\textwidth,
			enlarge x limits=0.05,,
			enlarge y limits={upper=0},
			xlabel={Maximum Number of Pebbles},
			xticklabels={9,10,11,12,13,14,15,16,17,23},
			ybar,
			axis y line*=left,
			bar width=4pt,
			legend style={at={(0.5,1.17)}, anchor=north,legend columns=-1},
			ylabel={No. obligations},
			x dir = reverse,
			fill between/on layer={main},
		]		
	        \legend{\ipdr o-count, naive o-count}
%	        \begin{filecontents}{ham7tc obligation-count.dat}
	        \pgfplotstableread{
	        	x y err
	            9 0.8 1.1242775458044156
	            10 130.6 21.567475512910637
	            11 67.3 19.87785199663183
	            12 44.6 8.10530690350464
	            13 36.6 5.199615370390391
	            14 29.6 10.799814813227124
	            15 32.714285714285715 12.426577367597496
	            16 29.666666666666668 7.748357054049396
	            17 33 0
	            19 193.5 6.002082971769051
	            % 23
	        }\oblcount
        	\errorbarplot{blue}{\oblcount};
%	        \begin{filecontents}{ham7tc naive obligation-count.dat}
			\pgfplotstableread{
	            x y err
	            9 12 0
	            10 372.6 28.83289787725126
	            11 375 45.21061822182926
	            12 300.6 29.362833650722475
	            13 268 10.16857905510893
	            14 248.3 11.933524207039595
	            15 232.57142857142858 16.047306159770955
	            16 241 4.08248290463863
	            17 231 0
	            19 193.5 6.002082971769051
	            % 23
	        }\noblcount
        	\errorbarplot{red}{\noblcount};
	        
      		\defxcrunch{0.11}{0.16}
      	\end{axis}
      
		\drawxcrunch

	    \begin{axis}
        [
			ymode=log,
			log origin=infty,
			xtick=data,
			xtick style={draw=none},
			x axis line style={draw=none},
			minor tick num=1,
			height=\plotheight,
			width=\textwidth,
			enlarge x limits=0.05,,
			enlarge y limits={upper=0},
			axis y line*=right,
			legend style={at={(0.5,1.04)}, anchor=north,legend columns=-1},
			xticklabels={,,},
%			ylabel={Time (s)},
			x dir = reverse,
			fill between/on layer={main},
		]
	        \legend{\ipdr o-time, naive o-time}
%	        \begin{filecontents}{ham7tc obligation-time.dat}
			\pgfplotstableread{
	            x y err
	            9 0.8202922705999999 1.2885606330432002
	            10 106.0217300456 27.66452546685597
	            11 36.1087847796 24.522193301870765
	            12 11.9647086355 3.6186424296488027
	            13 6.1279803073000005 1.7154989758489123
	            14 1.9904427260000002 1.008286755695432
	            15 1.1523403985714284 0.7376926638007634
	            16 1.120595703333333 0.4678302175091482
	            17 1.4657357190000002 0
	            19 3.9288569940000015 0.19449981237201608
	            % 23
	        }\obltime
	        \dotplot{blue}{\obltime};
		    \addplot [name path=upper,draw=none]
				table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\obltime};
			\addplot [name path=lower,draw=none] 
				table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\obltime};
			\filldevplot{blue}
%	        \begin{filecontents}{ham7tc naive obligation-time.dat}
			\pgfplotstableread{
	            x y err
	            9 3.5680185307000003 0.01813684335066361
	            10 189.29807288689992 28.54660661977086
	            11 112.19739899669999 40.50656380232495
	            12 44.868530388900005 13.668511095333836
	            13 14.682385296499998 3.8080319991172944
	            14 8.390014096000002 1.4128448844761268
	            15 6.577928030428572 0.5814390788171226
	            16 6.803558257333333 0.1774575614997469
	            17 5.989378324 0
	            19 3.9347875008999997 0.1952722059439133
	            % 23
	        }\nobltime
        \dotplot{red}{\nobltime};
	    \addplot [name path=upper,draw=none]
			table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\nobltime};
		\addplot [name path=lower,draw=none] 
			table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\nobltime};
		\linedevplot{red}
	    \end{axis}
	    %\caption{Statistics for ham7tc experiment.}
	    
	\end{tikzpicture}
\end{minipage}
%	\caption{
%	    Left axis: total number of obligations (obligation-count)
%	    handled by the minor iteration. Right axis: the time spent on
%	    them (obligation-time).
%	}\label{fig:pebbling:constrain:ham7:obl}
%	\end{subfigure}
%	
%		\begin{subfigure}{\textwidth}
%		\centering
	% Incremental times
\begin{minipage}{.5\textwidth}
	\begin{tikzpicture}		
		\begin{axis}
		[
			xtick=data,
			xtick style={draw=none},
			minor tick num=1,
			height=5cm,
			width=\textwidth,
			enlarge x limits=0.05,
			enlarge y limits={upper=0},
			xlabel={Maximum Number of Pebbles},
%			axis y line*=left,
			legend style={at={(0.5,1.23)}, anchor=north,legend columns=-1},
			ylabel={Time (s)},
			x dir = reverse,
			fill between/on layer={main},
		]
			\legend{\ipdr inc-time, naive inc-time}
%			\begin{filecontents}{ham7tc inc-time (constrain).dat}
			\pgfplotstableread{
				x y err
			    9 0.26132231679999995 0.03399652673484897
			    10 0.1215890968 0.0188224094715695
			    11 0.07217729329999999 0.007775473612871219
			    12 0.04853685640000001 0.00445019304784721
			    13 0.0336318478 0.0027108322124754537
			    14 0.028536875499999996 0.0034852225626870728
			    15 0.02628886714285714 0.0018837199875151615
			    16 0.024544915333333334 0.0024857351622102116
			    17 0.025080067 0
			}\inctime
			\dotplot{blue}{\inctime};
			\addplot [name path=upper,draw=none]
				table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\inctime};
			\addplot [name path=lower,draw=none] 
				table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\inctime};
			\filldevplot{blue}
%			\begin{filecontents}{ham7tc naive inc-time (constrain).dat}
			\pgfplotstableread{
				x y err
				9 0.0662037737 0.0009982932135989967
				10 0.06513288390000001 0.0007058335541635077
				11 0.064573517 0.0009061616199195369
				12 0.063899825 0.0007116947427317436
				13 0.0637975121 0.001095456718934567
				14 0.064155989 0.0017916209965402826
				15 0.06311204671428572 0.00015336877614961894
				16 0.06293949433333333 0.00015765172853546926
				17 0.062762295 0
			}\ninctime
		\dotplot{red}{\ninctime};
		\addplot [name path=upper,draw=none]
			table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\ninctime};
		\addplot [name path=lower,draw=none] 
			table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\ninctime};
		\linedevplot{red}
		\end{axis}
	\end{tikzpicture}
\end{minipage}

\begin{minipage}{.49\textwidth}
	\begin{tikzpicture}
	    \begin{axis}
			[
				 ymode=log,
				 log origin=infty,
				xtick={7,...,10},
				xtick style={draw=none},
				minor tick num=1,
				height=\plotheight,
				width=\textwidth,
				enlarge x limits=0.05,,
				enlarge y limits={upper=0},
				xlabel={Maximum Number of Pebbles},
				ybar,
				axis y line*=left,
					bar width=5pt,
				legend style={at={(0.5,1.23)}, anchor=north,legend columns=-1},
				ylabel={No. obligations},
				fill between/on layer={main},
			]		
	        \legend{\cipdr o-count, naive o-count}
%	        \begin{filecontents}{ham7tc obligation-count.dat}
	        \pgfplotstableread{
							x y err
							7 1 0
							8 7.8 0.681175454637056
							9 8.3 3.103063002905355
							10 424.9 69.22774732720978
	        }\oblcount
        	\errorbarplot{blue}{\oblcount};
%	        \begin{filecontents}{ham7tc naive obligation-count.dat}
					\pgfplotstableread{
							x y err
							7 1 0
							8 7.8 0.681175454637056
							9 12 0
							10 372.6 28.83289787725126
	        }\noblcount
        	\errorbarplot{red}{\noblcount};
      	\end{axis}

	    \begin{axis}
        [
          ymode=log,
          log origin=infty,
					xtick={7,...,10},
					xtick style={draw=none},
					minor tick num=1,
					height=\plotheight,
					width=\textwidth,
					enlarge x limits=0.05,,
					enlarge y limits={upper=0},
					axis y line*=right,
					legend style={at={(0.5,1.1)}, anchor=north,legend columns=-1},
					xticklabels={,,},
					ylabel={Time (s)},
					fill between/on layer={main},
				]
	        \legend{\cipdr o-time, naive o-time}
%	        \begin{filecontents}{ham7tc obligation-time.dat}
					\pgfplotstableread{
	            x y err
							7 0.0014916292999999998 0
							8 1.3327998512 0.12149405186689703
							9 3.0275430550999993 0.4908335124356978
							10 206.24312188169998 67.61955351235518
	        }\obltime
	        \dotplot{blue}{\obltime};
					\addplot [name path=upper,draw=none]
						table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\obltime};
					\addplot [name path=lower,draw=none] 
						table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\obltime};
					\filldevplot{blue}
%	        \begin{filecontents}{ham7tc naive obligation-time.dat}
					\pgfplotstableread{
	            x y err
							7 0.0014905496 0
							8 1.3328906591999998 0.12247734019036084
							9 2.1362515233999995 0.013411346549398682
							10 147.58029648619998 22.423577909455354
	        }\nobltime
        \dotplot{red}{\nobltime};
	    \addplot [name path=upper,draw=none]
			table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\nobltime};
		\addplot [name path=lower,draw=none] 
			table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\nobltime};
		\linedevplot{red}
	    \end{axis}
	    %\caption{Statistics for ham7tc experiment.}
	    
	\end{tikzpicture}
\end{minipage}
\begin{minipage}{.49\textwidth}
	\begin{tikzpicture}		
		\begin{axis}
			[
				ymin=0,
				xtick=data,
				xtick style={draw=none},
				minor tick num=1,
				height=5cm,
				width=0.8\textwidth,
				enlarge x limits=0.1,
				enlarge y limits={upper=0},
				ybar,
				axis y line*=right,
				xticklabels={,,},
				bar width=5pt,
				legend style={at={(0.5,1.26)}, anchor=north,legend columns=-1},
				ylabel={Copyrate (\%)},
				fill between/on layer={main},
			]
			\legend{\cipdr copyrate}
			% \begin{filecontents}{5bitadder relax-frames-perc (relax).dat}
			\pgfplotstableread{
					x y err
					8 0 0
					9 68.27586206896551 3.3786065417698965
					10 66.51378033730974 1.5513039743986192
			}\incperc
			\errorbarplot{blue}{\incperc};
		\end{axis}
	
		\begin{axis}
		[
%				ymax=8,
			xtick=data,
			xtick style={draw=none},
			minor tick num=1,
			height=5cm,
			width=0.8\textwidth,
			enlarge x limits=0.05,
			enlarge y limits={upper=0},
			xlabel={Maximum Number of Pebbles},
			axis y line*=left,
					legend style={at={(0.5,1.138)}, anchor=north,legend columns=-1},
%			ylabel={Time (s)},
			fill between/on layer={main},
		]
%			\begin{filecontents}{ham7tc inc-time (relax).dat}
			\pgfplotstableread{
				x y err
				8 0.0028068212 0.00014898600661995078
				9 0.014244686599999997 0.0009128519472177511
				10 0.025914295999999996 0.005760409145567388
			}\inctime
			\dotplot{blue}{\inctime};
			\addplot [name path=upper,draw=none]
				table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\inctime};
			\addplot [name path=lower,draw=none] 
				table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\inctime};
			\filldevplot{blue}
%			\begin{filecontents}{ham7tc naive inc-time (relax).dat}
			\pgfplotstableread{
			    x y err
					8 0.0634388488 0.0004648420572492997
					9 0.06239420130000001 0.0001754093652055396
					10 0.062633937 0.000277725819716858
			}\ninctime
		\dotplot{red}{\ninctime};
		\addplot [name path=upper,draw=none]
			table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\ninctime};
		\addplot [name path=lower,draw=none] 
			table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\ninctime};
		\linedevplot{red}
			\legend{\cipdr inc-time, naive inc-time}
		\end{axis}
	\end{tikzpicture}
\end{minipage}

%	\caption{
%		The amount of the runtime that was spent on copying clauses to the
%		constrained instance denoted on the x-axis. This number is already included
%		in the times of the upper graph. 
%	}
%	\label{fig:pebbling:constrain:ham7:inc}
%	\end{subfigure}
    \caption{
	    Statistics for the constraining (top) and relaxing (bottom) \texttt{ham7tc} experiment: obligation count (o-count), time (o-time), percentage clauses copied between \ripdr iterations and copy time (propagation time for \cipdr).
	    For 23 pebbles, \cipdr finds a trace with 18, so it continues with 17 pebbles (\autoref{l:forward}).
    }\label{fig:pebbling:constrain:ham7}
    \label{fig:stats}
\end{figure}

==> sections/experiments/results/stat-figures/ham7tc-constrain2.tex <==
{
\newcommand{\plotheight}{6cm}
	\begin{figure}[h]
	\centering
	\begin{subfigure}{\textwidth}
	\begin{tikzpicture}
	    \begin{axis}
		[
        	ymode=log,
			log origin=infty,
			xtick=data,
			xtick style={draw=none},
			x axis line style={draw=none},
			minor tick num=1,
			height=\plotheight,
			width=\textwidth,
			enlarge x limits=0.05,,
			enlarge y limits={upper=0},
			xlabel={Maximum Number of Pebbles},
			xticklabels={9,10,11,12,13,14,15,16,17,23},
			ybar,
			axis y line*=left,
			bar width=7pt,
			legend style={at={(0.5,1.17)}, anchor=north,legend columns=-1},
			ylabel={No. obligations},
			x dir = reverse,
			fill between/on layer={main},
		]		
	        \legend{\cipdr obligation-count, naive obligation-count}
%	        \begin{filecontents}{ham7tc obligation-count.dat}
	        \pgfplotstableread{
	        	x y err
	            9 0.8 1.1242775458044156
	            10 130.6 21.567475512910637
	            11 67.3 19.87785199663183
	            12 44.6 8.10530690350464
	            13 36.6 5.199615370390391
	            14 29.6 10.799814813227124
	            15 32.714285714285715 12.426577367597496
	            16 29.666666666666668 7.748357054049396
	            17 33 0
	            19 193.5 6.002082971769051
	            % 23
	        }\oblcount
        	\errorbarplot{blue}{\oblcount};
%	        \begin{filecontents}{ham7tc naive obligation-count.dat}
			\pgfplotstableread{
	            x y err
	            9 12 0
	            10 372.6 28.83289787725126
	            11 375 45.21061822182926
	            12 300.6 29.362833650722475
	            13 268 10.16857905510893
	            14 248.3 11.933524207039595
	            15 232.57142857142858 16.047306159770955
	            16 241 4.08248290463863
	            17 231 0
	            19 193.5 6.002082971769051
	            % 23
	        }\noblcount
        	\errorbarplot{red}{\noblcount};
	        
      		\defxcrunch{0.11}{0.16}
      	\end{axis}
      
		\drawxcrunch

	    \begin{axis}
        [
			ymode=log,
			log origin=infty,
			xtick=data,
			xtick style={draw=none},
			x axis line style={draw=none},
			minor tick num=1,
			height=\plotheight,
			width=\textwidth,
			enlarge x limits=0.05,,
			enlarge y limits={upper=0},
			axis y line*=right,
			legend style={at={(0.5,1.04)}, anchor=north,legend columns=-1},
			xticklabels={,,},
			ylabel={Time (s)},
			x dir = reverse,
			fill between/on layer={main},
		]
	        \legend{\cipdr obligation-time, naive obligation-time}
%	        \begin{filecontents}{ham7tc obligation-time.dat}
			\pgfplotstableread{
	            x y err
	            9 0.8202922705999999 1.2885606330432002
	            10 106.0217300456 27.66452546685597
	            11 36.1087847796 24.522193301870765
	            12 11.9647086355 3.6186424296488027
	            13 6.1279803073000005 1.7154989758489123
	            14 1.9904427260000002 1.008286755695432
	            15 1.1523403985714284 0.7376926638007634
	            16 1.120595703333333 0.4678302175091482
	            17 1.4657357190000002 0
	            19 3.9288569940000015 0.19449981237201608
	            % 23
	        }\obltime
	        \dotplot{blue}{\obltime};
		    \addplot [name path=upper,draw=none]
				table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\obltime};
			\addplot [name path=lower,draw=none] 
				table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\obltime};
			\filldevplot{blue}
%	        \begin{filecontents}{ham7tc naive obligation-time.dat}
			\pgfplotstableread{
	            x y err
	            9 3.5680185307000003 0.01813684335066361
	            10 189.29807288689992 28.54660661977086
	            11 112.19739899669999 40.50656380232495
	            12 44.868530388900005 13.668511095333836
	            13 14.682385296499998 3.8080319991172944
	            14 8.390014096000002 1.4128448844761268
	            15 6.577928030428572 0.5814390788171226
	            16 6.803558257333333 0.1774575614997469
	            17 5.989378324 0
	            19 3.9347875008999997 0.1952722059439133
	            % 23
	        }\nobltime
        \dotplot{red}{\nobltime};
	    \addplot [name path=upper,draw=none]
			table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\nobltime};
		\addplot [name path=lower,draw=none] 
			table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\nobltime};
		\linedevplot{red}
	    \end{axis}
	    %\caption{Statistics for ham7tc experiment.}
	    
	\end{tikzpicture}
	\caption{
	    Left axis: total number of obligations (obligation-count)
	    handled by the minor iteration. Right axis: the time spent on
	    them (obligation-time).
	}\label{fig:pebbling:constrain:ham7:obl}
	\end{subfigure}
	
		\begin{subfigure}{\textwidth}
		\centering
	% Incremental times
	\begin{tikzpicture}		
		\begin{axis}
		[
			xtick=data,
			xtick style={draw=none},
			minor tick num=1,
			height=4cm,
			width=0.8\textwidth,
			enlarge x limits=0.05,
			enlarge y limits={upper=0},
			xlabel={Maximum Number of Pebbles},
%			axis y line*=left,
			legend style={at={(0.5,1.23)}, anchor=north,legend columns=-1},
			ylabel={Time (s)},
			x dir = reverse,
			fill between/on layer={main},
		]
			\legend{\cipdr inc-time, naive inc-time}
%			\begin{filecontents}{ham7tc inc-time (constrain).dat}
			\pgfplotstableread{
				x y err
			    9 0.26132231679999995 0.03399652673484897
			    10 0.1215890968 0.0188224094715695
			    11 0.07217729329999999 0.007775473612871219
			    12 0.04853685640000001 0.00445019304784721
			    13 0.0336318478 0.0027108322124754537
			    14 0.028536875499999996 0.0034852225626870728
			    15 0.02628886714285714 0.0018837199875151615
			    16 0.024544915333333334 0.0024857351622102116
			    17 0.025080067 0
			}\inctime
			\dotplot{blue}{\inctime};
			\addplot [name path=upper,draw=none]
				table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\inctime};
			\addplot [name path=lower,draw=none] 
				table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\inctime};
			\filldevplot{blue}
%			\begin{filecontents}{ham7tc naive inc-time (constrain).dat}
			\pgfplotstableread{
				x y err
				9 0.0662037737 0.0009982932135989967
				10 0.06513288390000001 0.0007058335541635077
				11 0.064573517 0.0009061616199195369
				12 0.063899825 0.0007116947427317436
				13 0.0637975121 0.001095456718934567
				14 0.064155989 0.0017916209965402826
				15 0.06311204671428572 0.00015336877614961894
				16 0.06293949433333333 0.00015765172853546926
				17 0.062762295 0
			}\ninctime
		\dotplot{red}{\ninctime};
		\addplot [name path=upper,draw=none]
			table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\ninctime};
		\addplot [name path=lower,draw=none] 
			table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\ninctime};
		\linedevplot{red}
		\end{axis}
	\end{tikzpicture}
	\caption{
		The amount of the runtime that was spent on copying clauses to the
		constrained instance denoted on the x-axis. This number is already included
		in the times of the upper graph. 
	}
	\label{fig:pebbling:constrain:ham7:inc}
	\end{subfigure}

    \caption{
	    Statistics for the constraining \texttt{ham7tc} experiment,
	    averaged over 10 repetitions.
	    On constraint 23, the algorithm found a trace with 18 pebbles, so it could continue with constraint 17 afterwards.
    }\label{fig:pebbling:constrain:ham7}
\end{figure}
}

==> sections/experiments/results/stat-figures/ham7tc-relax.tex <==
{
\newcommand{\plotheight}{6cm}
	\begin{figure}[h]
	\centering
	\begin{subfigure}{\textwidth}
	\begin{tikzpicture}
	    \begin{axis}
			[
				 ymode=log,
				 log origin=infty,
				xtick={7,...,10},
				xtick style={draw=none},
				minor tick num=1,
				height=\plotheight,
				width=\textwidth,
				enlarge x limits=0.05,,
				enlarge y limits={upper=0},
				xlabel={Maximum Number of Pebbles},
				ybar,
				axis y line*=left,
				bar width=7pt,
				legend style={at={(0.5,1.17)}, anchor=north,legend columns=-1},
				ylabel={No. obligations},
				fill between/on layer={main},
			]		
	        \legend{\cipdr obligation-count, naive obligation-count}
%	        \begin{filecontents}{ham7tc obligation-count.dat}
	        \pgfplotstableread{
							x y err
							7 1 0
							8 7.8 0.681175454637056
							9 8.3 3.103063002905355
							10 424.9 69.22774732720978
	        }\oblcount
        	\errorbarplot{blue}{\oblcount};
%	        \begin{filecontents}{ham7tc naive obligation-count.dat}
					\pgfplotstableread{
							x y err
							7 1 0
							8 7.8 0.681175454637056
							9 12 0
							10 372.6 28.83289787725126
	        }\noblcount
        	\errorbarplot{red}{\noblcount};
      	\end{axis}

	    \begin{axis}
        [
          ymode=log,
          log origin=infty,
					xtick={7,...,10},
					xtick style={draw=none},
					minor tick num=1,
					height=\plotheight,
					width=\textwidth,
					enlarge x limits=0.05,,
					enlarge y limits={upper=0},
					axis y line*=right,
					legend style={at={(0.5,1.04)}, anchor=north,legend columns=-1},
					xticklabels={,,},
					ylabel={Time (s)},
					fill between/on layer={main},
				]
	        \legend{\cipdr obligation-time, naive obligation-time}
%	        \begin{filecontents}{ham7tc obligation-time.dat}
					\pgfplotstableread{
	            x y err
							7 0.0014916292999999998 0
							8 1.3327998512 0.12149405186689703
							9 3.0275430550999993 0.4908335124356978
							10 206.24312188169998 67.61955351235518
	        }\obltime
	        \dotplot{blue}{\obltime};
					\addplot [name path=upper,draw=none]
						table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\obltime};
					\addplot [name path=lower,draw=none] 
						table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\obltime};
					\filldevplot{blue}
%	        \begin{filecontents}{ham7tc naive obligation-time.dat}
					\pgfplotstableread{
	            x y err
							7 0.0014905496 0
							8 1.3328906591999998 0.12247734019036084
							9 2.1362515233999995 0.013411346549398682
							10 147.58029648619998 22.423577909455354
	        }\nobltime
        \dotplot{red}{\nobltime};
	    \addplot [name path=upper,draw=none]
			table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\nobltime};
		\addplot [name path=lower,draw=none] 
			table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\nobltime};
		\linedevplot{red}
	    \end{axis}
	    %\caption{Statistics for ham7tc experiment.}
	    
	\end{tikzpicture}
	\caption{
	    Left axis: total number of obligations (obligation-count)
	    handled by the minor iteration. Right axis: the time spent on
	    them (obligation-time). For constraint 7, no obligations were enqueued as \pdr terminated in the initialization step. Its obligation-count value was set to 1 to accommodate the logarithmic scale and the obligation-time to the total runtime (which is a close approximation).
	}\label{fig:pebbling:relax:ham7:obl}
	\end{subfigure}
	
	\begin{subfigure}{\textwidth}
		\centering
	% Incremental times
	\begin{tikzpicture}		
		\begin{axis}
			[
				ymin=0,
				xtick=data,
				xtick style={draw=none},
				minor tick num=1,
				height=4cm,
				width=0.8\textwidth,
				enlarge x limits=0.1,
				enlarge y limits={upper=0},
				ybar,
				axis y line*=right,
				xticklabels={,,},
				bar width=7pt,
				legend style={at={(0.52,1.45)}, anchor=north,legend columns=-1},
				ylabel={Copyrate (\%)},
				fill between/on layer={main},
			]
			\legend{\ipdr copyrate}
			% \begin{filecontents}{5bitadder relax-frames-perc (relax).dat}
			\pgfplotstableread{
					x y err
					8 0 0
					9 68.27586206896551 3.3786065417698965
					10 66.51378033730974 1.5513039743986192
			}\incperc
			\errorbarplot{blue}{\incperc};
		\end{axis}
	
		\begin{axis}
		[
			xtick=data,
			xtick style={draw=none},
			minor tick num=1,
			height=4cm,
			width=0.8\textwidth,
			enlarge x limits=0.05,
			enlarge y limits={upper=0},
			xlabel={Maximum Number of Pebbles},
			axis y line*=left,
			legend style={at={(0.52,1.23)}, anchor=north,legend columns=-1},
			ylabel={Time (s)},
			fill between/on layer={main},
		]
			\legend{\cipdr inc-time, naive inc-time}
%			\begin{filecontents}{ham7tc inc-time (relax).dat}
			\pgfplotstableread{
				x y err
				8 0.0028068212 0.00014898600661995078
				9 0.014244686599999997 0.0009128519472177511
				10 0.025914295999999996 0.005760409145567388
			}\inctime
			\dotplot{blue}{\inctime};
			\addplot [name path=upper,draw=none]
				table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\inctime};
			\addplot [name path=lower,draw=none] 
				table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\inctime};
			\filldevplot{blue}
%			\begin{filecontents}{ham7tc naive inc-time (relax).dat}
			\pgfplotstableread{
			    x y err
					8 0.0634388488 0.0004648420572492997
					9 0.06239420130000001 0.0001754093652055396
					10 0.062633937 0.000277725819716858
			}\ninctime
		\dotplot{red}{\ninctime};
		\addplot [name path=upper,draw=none]
			table[x=x,y expr=\thisrow{y}+\thisrow{err}] {\ninctime};
		\addplot [name path=lower,draw=none] 
			table[x=x,y expr=\thisrow{y}-\thisrow{err}] {\ninctime};
		\linedevplot{red}
		\end{axis}
	\end{tikzpicture}
	\caption{
		The amount of the runtime that was spent on copying clauses to the
		relaxed instance denoted on the x-axis. This number is already included
		in the times of the upper graph. 
	}
	\label{relax}
	\end{subfigure}

    \caption{
	    Statistics for the relaxing \texttt{ham7tc} experiment,
	    averaged over 10 repetitions.
    }\label{fig:pebbling:relax:ham7}
\end{figure}
}

==> tex/algorithm.tex <==
%%%%% 
% Main
%%%%%
\begin{algorithm}[p]
	\input{./tex/kw-definitions}
	\SetKwFunction{Fmain}{Main}
	\SetKwFunction{reduce}{Reduce}
	
	\Out{$\mathit{trace}$, series of board states that represent a path to a $P$-state}
	\Vars{$F$, the list of frames for the current run}
	\nthvar{$G$, the list of frames from a previous run}
	\;
	\SetKwProg{Fn}{function}{}{End}
	\Fn{\Fmain{$\trans[N]$}} {
		$n+1 \gets N; \quad$
		$k \gets 1$\;
		$F_0 \gets I;\quad \forall i > 0\colon F_i \gets \compl{P}$\;
		\lIf{$\exists i \in I \cap P$} { \Return{$i$} }
		\lIf{$\exists i \in I \cap T.P$} { \Return{$i,\ P$} }
		\While{$n > 0$}{
			$\condition{\trans[n] \subseteq \trans[{n+1}]}$\condend
			%
			\lIf{$n^\prime \neq \infty$}{\Fprop{$k$}}
			$\conditions
				{\forall 0 \leq i \le k,\ \forall c \in \blocked{F_i}\colon {\bf if }\ F_i.\trans[n] \subseteq \compl{c}^\prime\ {\bf then}\ c \not\in {F}_{i+1}\ ^*}
				{\trans[n] \subseteq T_{n+1}}
				{\assnp(G)}$\condend
			%
			$\conditions
				{\assn(F)}
				{\forall i > k + 1\colon F_i = \compl{P}}$\condend
			%
			${\it trace} \gets$ \Fstrategy{$\trans[n],\ k$}\;
			%
			$\conditions
				{\ \assn(F)}
				{{\bf if }\ {\it trace} = \varnothing\ {\bf then}\ F_k.\trans[n] \subseteq F^\prime_{k+1} }
				{\forall i > k + 1\colon F_i = \compl{P}}$\condend
			%
			\eIf{${\it trace} = \varnothing$}{
				\Return{\it strategy}\;
			}{
				$\condition{\mathit{trace} \text{ is a path to a } P \text{ state}}$\condend
					${\it strategy} \gets {\it trace}$\;
					$n^\prime \gets n$\;
					$n \gets n - 1$
			}
			$\conditions
				{\assnp(G)}
				{{\bf if }\ {\it trace} = \varnothing\ {\bf then}\ G_k.\trans[n] \subseteq G^\prime_{k+1} }
				{\forall i > k + 1\colon G_i = \compl{P}}$\condend
		}
	}
\algorithmfootnote{$^*$ Moet alleen als trace.}
\algpost{{\it trace} is a path to a $P$ state if it exists, for the smallest possible $n$}
\caption{Main loop, executing multiple runs of \pdr}
\end{algorithm}
%
%%%%%
% PDR
%%%%%
\begin{algorithm}
\caption{Determine whether the given model has a pebbling strategy}
%\SetAlgoLined
\input{./tex/kw-definitions}

\In{$\trans[n]$, transition relation under cardinality constraint $\cardclause{n}$}
\nthin{$F$, a series of Frames. $\varnothing$ or a list $F_0,\ F_1,\ \ldots,\ F_{\it last}$}
\Out{$\mathit{trace}$, series of states that represent a path to $P$}
\Globals{$I$, the initial state of the system}
\nthglob{$P$, the target state}
\algpre{$\conditions
        {\assn(F)}
        {\forall i > k + 1\colon \clauses{F_i} = \varnothing}$}
\;
\SetKwProg{Fn}{function}{}{End}
\Fn{\Fstrategy{$\trans[n],\ k$}} {
    \For{k \KwTo $\infty$}{
        $\conditions
            {\assn(F)}
            {\forall i > k + 1\colon F_i = \bar{P}}
            {\forall 0 \leq i < k, \forall c \in \blocked{F}{i}\colon {\bf if }\ F_i.\trans[n] \subseteq \bar{c}\ {\bf then}\ c \not\in {F}_{i+1}}$\condend
		\ForAll{$s \in F_k \cap \trans[n].P$}{
		    $\conditions
                {\assn(F)}
                {\forall c \in \blocked{F}{k+1}\colon F_k.\trans[n] \subseteq \bar{c} }
                {\forall i > k + 1\colon F_i = \bar{P}}$\condend
			${\it trace} \gets \Fblock{k-1,\ s,\ k}$\;
			\If{${\it trace} \neq \varnothing$}{
			    $\condition{\text{\it trace is a path to a P-state}}$\condend
  				\Return{\textit{trace}}
  			}
  		}\;
  		$\conditions
  		    {{\it trace} = \varnothing}
  		    {F_k.\trans[n] \subseteq F_{k+1}^\prime\ ^1}$\condend
		$F_{k+1} \gets \bar{P}$\;
		\Fprop{$k$}\;
		\If{$\exists 1 \leq i \leq k\colon F_i = F_{i+1}\colon$}
		{
			\Return{$\varnothing$}
		}
    }
}
\algorithmfootnote{$^1$ Since $F_{k+1} \equiv \bar{P}$ and all transitions to $\bar{P}$ have been removed.}
\algpost{$\conditions
    {\assn(F)}
    {\text{{\it trace} is a path to a $P$ state if it exists}}
    {{\bf if }\ {\it trace} = \varnothing\ {\bf then}\ F_k.\trans[n] \subseteq F_{k+1}}
    {\forall i > k + 1\colon F_i = \bar{P}}$}

\end{algorithm}
%
%%%%% 
% BLOCK
%%%%%
%
\begin{algorithm}
\caption{Try to eliminate a state as a potential path to $P$}
%\SetAlgoLined
\input{./tex/kw-definitions}
\SetKwProg{Fn}{function}{}{End}
\In{$i$, integer describing the level of a frame}
\nthin{$q$, a state that leads to $P$ in one transition}
\nthin{$k$, integer that is the current frontier of the main loop}
\algpre{$\conditions
        {\assn(F)}
        {\forall c \in \blocked{F}{k+1}\colon transdst{F_k} \subseteq \bar{c}^\prime }
        {\forall i > k + 1\colon F_i = \bar{P}}
        {0 < i \leq k+1 \land \ q \not\models F_i}
        {\notxinductiverelto{q}{F_{i-1}}} 
        {\exists\text{\it path from q to a P-state}}$}
                 
\Fn{\Fblock{$i,\ q,\ k$}} {
    ${\it obligations} \gets \set{(i,q)}$\;\;
    \While{$obligations \neq \varnothing$}{
        $\conditions
            {\bf Pre}
            {\forall (i,q) \in {\it obligations}\colon 0 < i \leq k+1 \land \ q \not\models F_i}
            {\forall (i,q) \in {\it obligations}\colon \notxinductiverelto{q}{F_{i-1}}} 
            {\forall (i,q) \in {\it obligations}\colon \exists\text{\it path from q to a P-state}}
            {\forall (i,q) \in {\it obligations_{prev}},\ \exists j \ge i\colon (j,q) \in {\it obligations}}$\condend
        $($\Int{} $n$, \Cube{} $s) := obligations$.\Ftop{}\;
    	\eIf{$\exists p \in F_n \cap \trans[n].{\set{s}}$}{
    		\If{$n = 0$}{ \Return{\it trace} }
    		$\conditions
    		    {p \not\models F_{\it n-1}}
    		    {\notxinductiverelto{p}{F_{n-2}}\ ^1}$\condend
     		${\it obligations} := {\it obligations} \cup \set{(n-1, p)}$\;
        } {
    		\Int{} $m :=$ \Fremove{$s,\ n+1,\ k$}\;
    		\If{$m < 0$}{ \Return{\it trace} }
    		${\it obligations} := {\it obligations} \setminus \set{(n,s)}$\;
    		\If{$m+1 \leq k$} { 
    		    $\conditions
    		        {s \not\models F_{\it m + 1}}
    		        {\notxinductiverelto{s}{F_m}\ ^2}$\condend
    			${\it obligations} := {\it obligations} \cup \set{(m+1,s)}$\;
    	    }
       }
    }
    \Return{$\varnothing$}
}

\algorithmfootnote{%
$^1$ If $\bar{p}$ were not inductive relative to $F_{n-2}$, then there is some $t \in F_{n-2}$ that is a predecessor to $p$, and by $\assn.4\colon p \in F_{n-1}$. But then $F_{n-1}$ would eventually lead to a $P$-state, which violates $\assn(F).3$ and $\assn(F).4$. Thus $\bar{p}$ is always inductive up to $F_{n-2}$.\\
$^2$ From \Fremove.
}


\algpost{$\conditions
    {{\bf if}\ {\it trace} \neq \varnothing\ {\bf then}\ \text{\it trace is a path to a P-state}}
    {\assn(F)}
    {\forall c \in \blocked{F}{k+1}\colon F_k.\trans[n] \subseteq \bar{c}^\prime }
    {\forall i > k + 1\colon F_i = \bar{P}}
    {\forall (i,q) \in {\it obligations}\colon q \not\models F_k}$}

\end{algorithm}
%
%%%%%%
% REMOVE
%%%%%%
%
\begin{algorithm}[p]
	\SetAlgoLined
	\input{./tex/kw-definitions}
	
	\Post{$s$ is excluded from all frames where $\compl{s}$ is inductive. }
	\Out{The highest such frame.}
	\algpre{$\conditions
		{\assn(F)}
		{\forall c \in \blocked{F_{k+1}}\colon F_k.\trans[n] \subseteq \compl{c}^\prime }
		{\forall i > k + 1\colon F_i = \compl{P}}
		{{\it min} \ge -1}
		{{\bf if}\ min \ge 0\ {\bf then}\ \notxinductiverelto{s}{F_{\it min}}}
		{\text{\it there is a path from s to a P-state}}$}
	
	\SetKwProg{Fn}{function}{:}{End}
	\Fn{\Fremove{$s: \Cube$, $min : \Int{}$}} {
		$m \gets k$\;
		\For{$i :=$ \Fmax{$0$, $min$} \KwTo $k$} {
			$\conditions
			{{\it min} < i \le k}
			{\forall 0 \le j < i\colon \notxinductiverelto{s}{F_j}}$\condend
			\If{$s \in (F_k \setminus s).\trans[n]$} {
				$m \gets i-1$\;
				\textbf{break}\;
			}
		}
		$\condition{\bf Pre}$\condend
		\eIf{$m \geq 0$} {
			$\condition{\notxinductiverelto{s}{F_m}}$\condend
			$c \gets S \ni s\ {\it such\ that\ } \notxinductiverelto{S}{F_m}$\;
			\For{$i:=1$ \KwTo $m+1$} {
				$F_i \gets F_i \setminus c$\; \alglabel{alg-remove-minus}		
			}
			$\condition{s \not\models F_{m+1}}$
		}{
			$\conditions
			{I \subseteq \compl{s}\ {\it and}\ (F_0 \setminus s).\trans[n] \not\subseteq \compl{s}^\prime}
			{(I \setminus s).\trans[n] \cap s^\prime \neq \varnothing}$\condend
			${\it trace} \gets i \in I,\ s,\ \ldots,\ P$
		}
		\Return{$m$}\;
	}
	\algpost{$\conditions
		{\assn(F)}
		{\forall c \in \blocked{F}{k+1}\colon F_k.\trans[n] \subseteq \compl{c}^\prime }
		{\forall i > k + 1\colon F_i = \compl{P}}
		{{\it min} \le m\le k}
		{{\bf if}\ m < 0\ {\bf then}\ \text{\it trace is a path from I to a P-state}}
		{{\bf if}\ m \ge 0\ {\bf then}\ s \not\models F_{\it m + 1}\ {\it and}\ \notxinductiverelto{s}{F_m}}$}
	
	\caption{Remove a state from all eligible frames.}
	\alglabel{alg-remove}
\end{algorithm}
%
%%%%%%
% PROPAGATE
%%%%%%
%
\begin{algorithm}
\input{./tex/kw-definitions}

\In{$k$, the frontier of the algorithm}
\algpre{$\conditions
  	    {\assn(F)}
  	    {\forall 0 \le i \le k\colon F_i.\trans[n] \subseteq F_{i+1}\ ^1}
  	    {\forall c \in \blocked{k+1}\colon F_k.\trans[n] \subseteq \bar{c} }
        {\forall i > k + 1\colon F_i = \bar{P}}$}

\SetKwProg{Fn}{function}{:}{End}
\Fn{\Fprop{$k$}} {
	\For{$i \gets 1\ \KwTo\ k$}{
	    $\condition{\forall 0 \leq j < i, \forall c \in \blocked{j}\colon {\bf if }\ F_i.\trans[n] \subseteq c\ {\bf then}\ c \in F_{j+1}}$\condend
		\ForAll{$c \in \blocked{i}$}{
		    $\condition{\bf Pre}$\condend
		    \If{$F_i.\trans[n] \not\ni c$}{
		        $F_{i+1} \gets F_{i+1} \setminus c$\;	\alglabel{alg-prop-minus}
		    }
		}
	}
}

\algorithmfootnote{$^1$ From $\assn(F).4$ and ${F_k.\trans[n] \subseteq F_{k+1}}$}

\algpost{$\conditions
        {\assn(F)}
        {\forall c \in \blocked{k+1}\colon F_k.\trans[n] \subseteq \bar{c}}
        {\forall 0 \le i \le k\colon F_i.\trans[n] \subseteq F_{i+1}}
        {\forall i > k + 1\colon F_i = \bar{P}}
        {\forall 0 \leq i \leq k, \forall c \in \blocked{i}\colon {\bf if }\ F_i.\trans[n] \subseteq \bar{c}\ {\bf then}\ c \not\in {F}_{i+1}}$}
\caption{Propagate any clauses that hold at higher levels}
\alglabel{alg-prop}
\end{algorithm}

==> tex/algorithms/case/peterson.tex <==
\begin{algo}[t]
    \caption{The Peterson algorithm for mutual exclusion for $n > 2$ processes, or the Filter lock \cite{peterson, peterson2}.}
    
    \newcommand{\Arr}[2]{\ensuremath{\mathit{#1}[#2]}}
    \newcommand{\alg}{alg:ipdr:peter}
    \label{\alg}
    
    \In{$n$, an integer denoting the number of processes.}
    \Vars{ $0 \le p < n$, an integer indicating the current process-id.\newline
        \textit{level}, an array of $n$ integers\newline
        \textit{last}, an array of $n-1$ integers}

\SetKwFunction{Fpeter}{Peterson-lock}
\SetKwFunction{Fpeterrelease}{Peterson-unlock}
\func{void}{\Fpeter{$n$}} {
    \For{$\Arr{level}{p} \gets 0$ \KwTo $n-2$ \label{\alg:loop}}
    {
        $\Arr{last}{\Arr{level}{p}} \gets p$\;    
        \While{$\Arr{last}{\Arr{level}{p}} = p \spaced\land \exists k \neq p\colon \Arr{level}{k} \ge \Arr{level}{p}$} 
        { \textbf{nothing} }
    }
    $\Arr{level}{p} \gets n-1\quad$  \codecomment{p is in the critical section}
}

\func{void}{\Fpeterrelease{}} {
    \ttfunction{assert}[$\Arr{level}{p} = n-1$]\;
    $\Arr{level}{p} \gets -1$;
}

\end{algo}


==> tex/algorithms/graph.tex <==
\begin{algo}[ht]
    \caption{A simple graph search algorithm} 
    \input{./tex/kw-definitions}

    \newcommand{\alg}{ex:intro:graph}

	\label{\alg}

	\In{
			A sequence $\nary{F_0, F_1, \ldots, F_{k+1}}$ and transition system \ts
			from the \pdr-state from \autoref{def:pdr-state}.	
	}

\func{\Void}{\Fpeter{$p$}} {
  $\mathit{level} \gets \Int[p]$ \;
  $\mathit{last} \gets \Int[p-1]$ \;
}
\end{algo}



==> tex/algorithms/imp/subsume.tex <==
\begin{algo}[t]
	\caption{Removing cube and removing any subsumed cubes. Note that while the implementation uses the delta-encoding from \autoref{imp:delta}, this listing uses the full semantics of $B$ and not the encoding. } 
	
	\newcommand{\alg}{alg:imp:subsume}
	
	\label{\alg}
	
	\In{%
		$F = \set{F_0, F_1, \ldots F_k}$, a sequence of candidates (\autoref{def:frames}). \newline
		$B = \set{B_1, B_2, \ldots B_k}$, a series of sets representing blocked states in $F$ (\autoref{def:blocked}). \newline
		$\form S$, representing a set of states $S$. \newline
		$l$, describing the candidates $\nary{F_1, F_2, \ldots F_l}$ that \form S is to be removed from.
	}
	
	\func{\Void}{\Fsubsume{$F,\ B,\ \form S,\ l$}} {
		\For{$i \gets 1$ \KwTo $l$}{
			$B_i \gets \set{\form C \in B_i \mid \textbf{not}\ \form S\ \mathit{subsumes}\ \form C}$\;
		}
	
		\For{$i \gets 1$ \KwTo $l$} {
			$\form F_i \gets \form F_i \land \neg\form S$\;
			$\blocked{i} \gets \blocked{i} \cup \form S$\;
		}
	}
\end{algo}

==> tex/algorithms/ipdr/constrain-loop.tex <==
\begin{algo}[t]
    \caption{Loop to verify a monotonically decreasing series of instances} 
    \input{./tex/kw-definitions}

    \newcommand{\alg}{alg:ipdr:constrain-loop}

	\label{\alg}

	\In{
			A sequence $\nary{F_0, F_1, \ldots, F_{k+1}}$ and transition system \ts
			from the \pdr-state from \autoref{def:pdr-state}.	
	}

  \newcommand{\result}{\ensuremath{\mathit{result}}}

\func{\Void}{\Fipdrconstrainloop{$\ts,\ P$}} {

    \lIf{$I \not\subseteq P$}{ \label{\alg:0}
        \Return{$\vec i \in I \cap \compl P$}
    }
    \lIf{$I.\trans \not\subseteq P$}{ \label{\alg:1}
        \Return{$\pair{\vec i}{\vec p} \in \fromto{I}{\compl P}$}
    }
    $\nary{F_0 \gets I, F_1 \gets P, F_2 \gets P}$\;  \label{\alg:init}
    $k \gets 1$\;
    $O \gets \set{}$ \;

  \While{$\result \neq \varnothing$}{

    $\result \gets \Fipdrmain{\nary{F, k, O, \ts, P}}$\;

    $\ts\constrained \gets\ $  \textit{reduce} \ts\;

    $\tuple{F, k, O, \ts, P} \gets %
    \ttfunction{ipdr-constrain}[\tuple{F, k, O, \ts, P}, I\constrained, \trans\constrained]$
  }
}
\end{algo}



==> tex/algorithms/ipdr/ipdr-constrain.tex <==
\begin{algo}[t]
    \input{./tex/kw-definitions}
    
    \newcommand{\alg}{alg:ipdr:constrain}
    \caption{The outer loop for constraining Incremental \pdr}
    \label{\alg}
    
    \In{$\mathit{TS} = \tsystem$, a tuple representing a transition system \newline 
        $P$, a property to be checked for invariance under $M$
    }
    
    \func{\Trace}{\Fipdrconstrain{$M,\ P$}} {
        \lIf{$\exists\vec i \in I \cap \compl P$}{ \label{\alg:0}
            \Return{$\vec i$}
        }
        $\nary{F_0 \gets I, F_1 \gets P, F_2 \gets P}$\;  \label{\alg:init}
        $k \gets 1$\;
        
        \While{$\mathit{trace} \neq \varnothing$}
        {
            \eIf{$\exists\pair{\vec i}{\vec p} \in \fromto{I}{\compl P}$ \label{\alg:1}}
                { \textit{trace} {$\gets \pair{\vec i}{\vec p}$} }
                { $\mathit{trace} \gets$ \Fipdrmain{$\nary{F, k, \varnothing, TS, P}$} }
            $TS \gets \tuple{2^X, I, \trans\constrained}$\;
        }
        \Return{\textit{trace}}
    }
\end{algo}



==> tex/algorithms/ipdr/ipdr-main.tex <==
\begin{algo}[t]
%\input{./tex/kw-definitions}

\newcommand{\alg}{alg:ipdr:main}
\caption{The modified major loop for Incremental \pdr}
\label{\alg}

\Pre{
	\Fprop and \Oprop.
}

\In{A tuple $\tuple{F, k, O, \ts, P}$, as defined in \autoref{def:pdr-state}
}

\func{\Trace}{\Fipdrmain{$\nary{F, k, O, \ts, P}$}} {
    
    \For{$k$ \KwTo $\infty$}{ \label{\alg:for}
        \ForAll{$\pair{\vec{o}}{\vec p} \in \fromto{F_k}{\compl P}$}{ \label{\alg:cti-query} \label{\alg:entry}	
			{\it trace} $\gets$ \Fblock{$\pair{\vec o}{k-1}$, $k$}\; \label{\alg:minor} 	
			\If{${\it trace} \neq \varnothing$}{
  				\Return{\textit{trace}}
  			}
  		}
		$F_{k+2} \gets P$\;
		\Fpropa{$F, k, \ts$}\; \label{\alg:prop}
		\If{$\exists 1 \leq i \leq k\colon F_i = F_{i+1}\colon$}
		{
			\Return{$\varnothing$}
		}
    }
}

\Out{\textit{trace}: a counter-example to the invariance of $P$ if it exists}
\end{algo}


==> tex/algorithms/ipdr/ipdr-relax.tex <==
\begin{algo}[t]
\input{./tex/kw-definitions}

\newcommand{\alg}{alg:ipdr:relax}
\caption{The outer loop for relaxing Incremental \pdr}
\label{\alg}

\In{$\mathit{TS} = \tsystem$, a tuple representing a transition system \newline 
    $P$, a property to be checked for invariance under $M$
}

\func{\Trace}{\Fipdrrelax{$TS,\ P$}} {
    \lIf{$\exists\vec i \in I \cap \compl P$}{ \label{\alg:0}
        \Return{$\vec i$}
    }
    \lIf{$\exists\pair{\vec i}{\vec p} \in \fromto{I}{\compl P}$}{ \label{\alg:1}
        \Return{\textit{trace} {$\gets \pair{\vec i}{\vec p}$}}
    }

    $\nary{F_0 \gets I, F_1 \gets P, F_2 \gets P}$\;  \label{\alg:init}
    $k \gets 1$\;

    \newcommand{\prev}{\ensuremath{\mathit{trace}_\mathit{prev}}}
    
    \While{$\mathit{trace} = \varnothing$}
    {
        $\prev \gets \mathit{trace}$\;
        $\mathit{trace} \gets$ \Fipdrmain{$\nary{\Fipdrprep{F}, 1, \varnothing, TS, P}$}\;
        $TS \gets \tuple{2^X, I, \trans\relaxed}$\;
    }
    \Return{\prev}
}

\end{algo}

==> tex/algorithms/ipdr/prepare.tex <==
\begin{algo}[t]
    \caption{The extraction of all cubes in a sequence of candidates that are reachable in one step under \textit{TS}} 
    \input{./tex/kw-definitions}

    \newcommand{\alg}{alg:ipdr:prep}

	\label{\alg}
	
	\In{$\mathit{TS} = \tsystem$, a tuple representing a transition system}
    
    \func{\Candidates}{\Fipdrprep{$\nary{\mathit{TS}, F\colon \Candidates}$}} {
        \ForAll{$\form C \in \blocked{1}$}{
    		\If{$\form I \land \trans \implies \neg\form C$} {
      			$\form F\primed_{1} \gets \form F\primed_{1} \land \neg\form C$\;
      			$B\primed_1 \gets B\primed_{1} \cup \form C$\;
      		}
      	}
      \Return{$\set{\nary{I, F\primed_i}}$}
}
\end{algo}

==> tex/algorithms/ipdr/relax-loop.tex <==
\begin{algo}[t]
    \caption{Loop to verify a monotonically increasing series of instances} 
    \input{./tex/kw-definitions}

    \newcommand{\alg}{alg:ipdr:relax-loop}

	\label{\alg}

	\In{
			A sequence $\nary{F_0, F_1, \ldots, F_{k+1}}$ and transition system \ts
			from the \pdr-state from \autoref{def:pdr-state}.	
	}

  \newcommand{\result}{\ensuremath{\mathit{result}}}

\func{\Void}{\Fipdrrelaxloop{$\ts,\ P$}} {

    \lIf{$I \not\subseteq P$}{ \label{\alg:0}
        \Return{$\vec i \in I \cap \compl P$}
    }
    \lIf{$I.\trans \not\subseteq P$}{ \label{\alg:1}
        \Return{$\pair{\vec i}{\vec p} \in \fromto{I}{\compl P}$}
    }
    $\nary{F_0 \gets I, F_1 \gets P, F_2 \gets P}$\;  \label{\alg:init}
    $k \gets 1$\;
    $O \gets \set{}$ \;

  \While{$\result = \varnothing$}{

    $\result \gets \Fipdrmain{\nary{F, k, O, \ts, P}}$\;

    $\ts\relaxed \gets\ $  \textit{increase} \ts\;

    $\tuple{F, k, O, \ts, P} \gets %
    \ttfunction{ipdr-relax}[\tuple{F, k, O, \ts, P}, I\relaxed, \trans\relaxed]$
  }
}
\end{algo}




==> tex/algorithms/major.tex <==
\begin{algo}[t]
\caption{The major iteration of \pdr}
\input{./tex/kw-definitions}

\newcommand{\alg}{alg:pdr:major}
\label{\alg}

\In{
  A transition system \ts and a property $P$.
}

\func{}{\Fpdr{$\ts,\ P$}} {
    \lIf{$I \not\subseteq P$}{ \label{\alg:0}
        \Return{$\vec i \in I \cap \compl P$}
    }
    \lIf{$I.\trans \not\subseteq P$}{ \label{\alg:1}
        \Return{$\pair{\vec i}{\vec p} \in \fromto{I}{\compl P}$}
    }
    $\nary{F_0 \gets I, F_1 \gets P, F_2 \gets P}$\;  \label{\alg:init}
    \For{$k \gets 1$ \KwTo $\infty$}{ \label{\alg:for}

        \ForAll{$\pair{\vec{o}}{\vec p} \in \fromto{F_k}{\compl P}$}{ \label{\alg:cti-query} \label{\alg:query} \label{\alg:entry}

			{\it trace} $\gets$ \Fblock{$F,\ k,\ \set{\pair{\vec o}{k-1}},\ \ts,\ P$}\; \label{\alg:minor} 	

			\If{${\it trace} \neq \varnothing$}{
  				\Return{\textit{trace}}
  			}
            \codecomment{$\vec o \not\in F_k$}
  		}
		$F_{k+2} \gets P$\; \label{\alg:push}
		\Fpropa{$\nary{F, k, \ts}$}\; \label{\alg:prop}
		\If{$\exists 1 \leq i \leq k\colon F_i = F_{i+1}\colon$ \label{\alg:fixpoint}} 
		{
			\Return{$\varnothing$}
		}
    }
}

\Out{\textit{trace}, a counter-example to the invariance of $P$ if it exists}
\end{algo}


==> tex/algorithms/mic.tex <==
\begin{algo}[t] 
    \caption{Find a minimal inductive subclause}
	
	\newcommand{\alg}{alg:pdr:generalize}
	\label{\alg}
	
	\In{
		A state \vec s, one of the candidates $F_i$ and a transition system \ts.
	}
	\Pre{\vec s is inductive relative to $F_{i}$.}

    \SetKwFunction{Fdrop}{drop}
    \SetKwFunction{Flits}{lits}

	\func{\Cube{}}{\Fmic{$\vec s$, $F_i$}} {
	    $\form C \gets \nary[\land]{s_1, s_2, \ldots}$\;
		\For{$l \in \form C$} {
		    $\form S \gets$ \Fdown{$\form C \setminus l,\ F_i,\ \ts$}\;
			\If{$\form S \neq \mathit{failure}$} {
				$\form C \gets \form S$
			}
		}
		\Return{$\form C$}
	}
	
	\Post{An inductive cube \form C that contains a subset of the literals in $\vec s$:\newline
        $\eform s \implies C$, $\form I \implies \neg \form C$ and \negindB{i}{C}}
\end{algo}
	
\begin{algo}[t] 
	\caption{
		The \texttt{down} \cite{down} algorithm to validate a cube with a dropped
		literal from \texttt{generalize}.
	}

	\In{
		A cube $\form C$, representing a set of states, a candidate $F_i$ and a
		transition system \ts. Where $F_i$ has a boolean representation $\form F_i$
		and \ts has a boolean representation $\form I$ for its initial states and
		$\form T$ for its transition relation respectively.
	}
	
	\newcommand{\alg}{alg:pdr:down}
	\label{\alg}
	
	\func{\Cube}{\Fdown{$\form C$, $F_i,\ \ts$}} {
        $\form S \gets \form C$\;
		\Loop{}{
		    \If{$\form I \not\implies \neg \form S$ \label{\alg:init}} 
		    { \Return{\textit{failure}} \label{\alg:none} } 
		    
		  %  \eIf{$\form F_i \land \neg \form C \land \trans \implies \form \neg C\primed$}
		    \eIf{\negindB{i}{\form S} \label{\alg:query}} 
		    { \Return{$\form S$}\; }
		    {
		      $\eform q \gets$ \textit{a witness such that } $\eform q \implies \form F_i \land \neg\form S$ \textit{ and } $\eform q \land \transf \land \form S\primed$\;
		      $\form S \gets$ \textit{a cube of all literals l, such that} $l \in \form S \land l \in \eform q$ \; \label{\alg:inter}
		    }
		}
	}

	\Post{An inductive subcube $\form S$ of the original $\form C$:\newline
         $\form C \implies S$, $\form I \implies \neg \form S$ and $\negindB{i}{S}$. \newline
			 Or \textit{failure} if no such cube exists.}
\end{algo}


==> tex/algorithms/minor.tex <==
\begin{algo}[t]
    \caption{The minor iteration of \pdr}
    
    \newcommand{\alg}{alg:pdr:minor}
    \label{\alg}
    
\In{A tuple \statetuple as defined in \autoref{def:pdr-state},\newline 
    thus \ts is a tuple \tsystem.}

\Pre{
  $O = \set{\pair{\vec o}{k-1}}$, where \vec o must be proven unreachable in
  $k$ steps or \invprop fails:\newline
     \cvec o \textit{is inductive relative to} $F_{i-1}\colon \vec o
     \not\in (F_{i-1}\setminus\vec o).\trans$,\newline
     $\exists \pair{\vec o}{\vec p} \in \trans\colon \vec p \not\in P$
}
    

\func{\Trace}{\Fblock{\stateargs}} {

    \While{$O \neq \varnothing$}{ \label{\alg:loop}

        $\pair{\vec s}{n} \gets O\ttfunction{.front}[]$ \hfill \codecomment{$\forall \pair{\vec q}{i} \in O\colon n\le i$}\;

        \eIf{$\exists \vec{p} \in F_n \colon\ \trans\pair{\vec p}{\vec s}$}{ \label{\alg:query}

            \If{$n = 0$}{ \label{\alg:init}

  			    \Return{a path from \vec p to a non-$P$-state}
  		    }

  			$O \gets O \cup \pair{\vec p}{n-1}$\; \label{\alg:rec}
  		}

  		{\label{\alg:else}
        $m \gets$ \Fremove{$\nary{\vec{s}, n, F, k, \ts}$}\; \label{\alg:remove}
      		$O \gets O \setminus \pair{\vec s}{n}$\hfill \codecomment{$ {\vec s} \not\in F_{n+1}$}\; \label{\alg:dequeue}
      		\If{$m+1 \le k$ \label{\alg:boundcheck}}{
      		    $O \gets O \cup \pair{\vec s}{m+1}$\; \label{\alg:push}
      		}
  		}
    }
    \Return{$\varnothing$}
}

\Post{\Fprop\newline 
        if $trace = \varnothing$, then $\vec o \not\in F_k$ and for all $\vec s$ that were enqueued on \cref{\alg:rec} and \ref{\alg:push}: $\vec s \not\in F_k$.}
\Out{\textit{trace}, a counter-example to \invprop if it exists.}
\end{algo}


==> tex/algorithms/peterson.tex <==
\begin{algo}[ht]
    \caption{Peterson's protocol for mutual exclusion \cite{peterson}} 
    \input{./tex/kw-definitions}

    \newcommand{\alg}{ex:intro:peterson}

	\label{\alg}

  \newcommand{\id}{\ensuremath{\mathit{id}}}
  \newcommand{\level}{\ensuremath{\mathit{level}}}
  \newcommand{\last}{\ensuremath{\mathit{last}}}

	\In{%
    An integer $\id$, representing the process id of the current
    process.\newline
    An integer $p$, representing the total number of processes that share a
    resource.
	}

\func{\Void}{\Fpeter{$\id,\ p$}} {
  $\level \gets \Int[p]$ \;
  $\last \gets \Int[p-1]$ \;

  \For{$l \gets 0\ \KwTo\ p-1$}{
    
    $\level[\id] \gets l$\;
    $\last[l] \gets \id$\;

      \While{
        $\last[l] = \id \land 
         \exists k \neq \id\colon \level[k] \ge l$
       }{
         \textbf{wait}\;
       }
  }
  
  \codecomment{Critical section}
}
\end{algo}


==> tex/algorithms/reach.tex <==
\begin{algorithm}[t]
\caption{Single step reachability check for incremental \pdr}
\input{./tex/kw-definitions}
\newcommand{\alg}{alg:pdr:reach}
	\label{\alg}

\SetKwFunction{Freach}{reach}
\SetKwProg{Fn}{function}{:}{End}
\nonl\Fn{\Freach{$F$}} {
    $F_{new} \gets P$\;
    \ForAll{$C \in \texttt{blocked(} F\texttt{)}$}{
		\If{$I \subseteq \compl C$ and $I.\trans \subseteq \compl C$} { 
  			$F_{new} \gets F_{new} \setminus C$\;
  		}
  	}
  	\Return{$F_{new}$}
}
\end{algorithm}

==> tex/algorithms/remove.tex <==
\begin{algo}[t]
	
	\newcommand{\alg}{alg:pdr:remove}
	\caption{Remove a state from all eligible frames.}
	\label{\alg}

    \In{
			${\vec s}\in S$: a state that can be blocked in \frames[i+1];\newline
			${i} \in \Natural$: the level of candidate to which $\cvec s$ is
			inductive.\newline
			A sequence $\nary{F_0, F_1, \ldots, F_{k+1}}$ and transition system \ts
			from the \pdr-state from \autoref{def:pdr-state}.	
		}
	\Pre{$i > 0$; \newline
         $\vec s \not\in (F_{i}\setminus\vec s).\trans$;\newline  
         $\exists \pi = \nary{\vec s, \pi_1, \pi_2, \ldots, \pi_n \not\in P}$.}
	
	\func{\Int}{\Fremove{${\vec s}\colon \State,\ {i}\colon \Int,\ F,\ k,\ \ts$}} {

		\For{$i \gets i+1$ \KwTo $k$} { \label{\alg:push} \label{\alg:for}
			\If{$\vec s \in (F_i \setminus \vec s).\trans$} { \label{\alg:ind}
			    $m \gets i-1$\;
				\textbf{break}\;
			}
		}

		$\form C \gets$ \Fgen{$\nary{\vec s, m, F, k, \ts}$}\; \label{\alg:gen} \label{\alg:generalize}

		\For{$i \gets 1$ \KwTo $m+1$} {
		    $\form F_i \gets \form F_i \land \neg\form C$\; \label{\alg:remove} 	
			$\blocked{i} \gets \blocked{i} \cup \form C$\; \label{\alg:blocked}
		}
		\Return{$m$}\;
	}
	
	\Post{$\vec s$ is inductive relative to $F_{m}$ and is excluded from \frames[m+1]; where $m \le k$}
	\Out{The highest candidate $F_m$ for which $\vec s \not\in (F_m\setminus\vec s).\trans$.}
	
\end{algo}


==> tex/example/constrain-example.tex <==
 \begin{figure}[ht] 
        \centering 
        \begin{subfigure}{0.4\textwidth}
            \begin{tikzpicture}
                \node[draw, circle] at (0,0)  (a) [initial] {$a$};
                \node[draw, circle] at (1,0)  (b) {$b$};
                \node[draw, circle] at (2,0)  (c) {$c$};
                \node[draw, circle] at (3,0)  (d) {$d$};
                \node[draw, circle] at (3,-1) (e) [accepting] {$e$};
                
                %Lines
                \draw[->] (a) edge (b);
                \draw[->] (b) edge (c);
                \draw[->] (c) edge (d);
                \draw[->] (d) edge (e);
            \end{tikzpicture}
						\caption{\textit{Simple}}
        \end{subfigure}
        \vspace{1em}

        \begin{subfigure}{0.4\textwidth}
            \begin{tikzpicture}
                \node[draw, circle] at (0,0)  (a) [initial] {$a$};
                \node[draw, circle] at (1,0)  (b) {$b$};
                \node[draw, circle] at (2,0)  (c) {$c$};
                \node[draw, circle] at (3,0)  (d) {$d$};
                \node[draw, circle] at (3,-1) (e) [accepting] {$e$};
                
                %Lines
                \draw[->] (a) edge (b);
                \draw[->] (c) edge (d);
                \draw[->] (d) edge (e);
            \end{tikzpicture}
        \caption{\textit{Simple}$\constrained$}
        \end{subfigure}
        \caption{Two instances of a \textit{Simple} system.}
        \label{ex:ipdr:constrain}
\end{figure}



==> tex/example/delta-encoding.tex <==
\[
\begin{array}{lll}
     \multicolumn{3}{c}{\bf Normal\ B} \\
     B_1 & B_2 & B_3 \\\hline
     a & a & \\
     b & b & b \\
     c
\end{array}\quad
\begin{array}{lll}
    \multicolumn{3}{c}{\bf Delta-B} \\
    B_1 & B_2 & B_3 \\\hline
     & a & \\
     &  & b \\
    c
\end{array}
\]

==> tex/example/relax-example.tex <==
 \begin{figure}[ht] 
        \centering 
        \begin{subfigure}{0.4\textwidth}
            \begin{tikzpicture}
                \node[draw, circle] at (0,0)  (a) [initial] {$a$};
                \node[draw, circle] at (1,0)  (b) {$b$};
                \node[draw, circle] at (2,0.5)  (c) {$c$};
                \node[draw, circle] at (2,-0.5)  (d) {$d$};
                \node[draw, circle] at (3,0) (e) [accepting] {$e$};
                
                %Lines
                \draw[->] (b) edge (c);
                \draw[->] (b) edge (d);
                \draw[->] (c) edge (e);
                \draw[->] (d) edge (e);
            \end{tikzpicture}
						\caption{\textit{Simple}}
        \end{subfigure}
        \vspace{1em}

        \begin{subfigure}{0.4\textwidth}
            \begin{tikzpicture}
                \node[draw, circle] at (0,0)  (a) [initial] {$a$};
                \node[draw, circle] at (1,0)  (b) {$b$};
                \node[draw, circle] at (2,0.5)  (c) {$c$};
                \node[draw, circle] at (2,-0.5)  (d) {$d$};
                \node[draw, circle] at (3,0) (e) [accepting] {$e$};
                
                %Lines
                \draw[->] (a) edge (b);
                \draw[->] (b) edge (c);
                \draw[->] (b) edge (d);
                \draw[->] (c) edge (e);
                \draw[->] (d) edge (e);
            \end{tikzpicture}
        \caption{\textit{Simple}$\relaxed$}
        \end{subfigure}
        \caption{Two instances of a \textit{Simple} system.}
        \label{ex:ipdr:relax}
\end{figure}




==> tex/figures/relaxing.tex <==
\begin{figure}[t]
        \centering 
        \begin{subfigure}{0.4\textwidth}
            \begin{tikzpicture}
                \node[draw, circle] at (0,0) (a) [initial] {$a$};
                \node[draw, circle] at (2,0) (b) {$b$};
                \node[draw, circle] at (2,-1) (c) {$c$};
                \node[draw, circle] at (0,-1) (d) {$d$};
                
                %Lines
                \draw[->] (a) edge[bend left=30] (b);
                \draw[->] (a) edge (d);
                \draw[->] (b) edge[bend left=30] (a);
                \draw[->] (b) edge (c);
            \end{tikzpicture}
        \caption{$\trans$}
        \end{subfigure}
        \begin{subfigure}{0.4\textwidth}
            \begin{tikzpicture}
                \node[draw, circle] at (0,0) (a) [initial] {$a$};
                \node[draw, circle] at (2,0) (b) {$b$};
                \node[draw, circle] at (2,-1) (c) {$c$};
                \node[draw, circle] at (0,-1) (d) {$d$};
                
                %Lines
                \draw[->] (a) edge[bend left=30] (b);
                \draw[->] (a) edge (d);
                \draw[->] (b) edge[bend left=30] (a);
                \draw[->] (b) edge (c);
                \draw[->] (c) edge[bend left=30] (d);
                \draw[->] (d) edge[bend left=30] (c);
            \end{tikzpicture}
        \caption{$\trans\relaxed$}
        \end{subfigure}
        \caption{Relaxing example: monotonically increasing $\trans$.}
        \label{fig:ipdr:relax}
\end{figure}

==> tex/front/abstract.tex <==
\begin{abstract}
    

\end{abstract}

\cleardoublepage

==> tex/front/title-page.tex <==
% \newgeometry{
% 	paper=a4paper, % Change to letterpaper for US letter
% 	inner=2.5cm, % Inner margin
% 	outer=3.8cm, % Outer margin
% 	bindingoffset=.5cm, % Binding offset
% 	top=1.5cm, % Top margin
% 	bottom=1.5cm, % Bottom margin
% 	%showframe, % Uncomment to show how the type block is set on the page
% }

\begin{titlepage}
\begin{center}

\vspace*{-0.06\textheight}
{\scshape\LARGE \univname\par}\vspace{1.5cm} % University name
\textsc{\Large Master's Thesis}\\[0.5cm] % Thesis type

\HRule \\[0.4cm] % Horizontal line
{\huge \bfseries \ttitle\par}\vspace{0.4cm} % Thesis title
\HRule \\[1.5cm] % Horizontal line
 
\begin{minipage}[t]{0.4\textwidth}
\begin{flushleft} \large
\emph{Author:}\\
\authorname % Author name - remove the \href bracket to remove the link
\end{flushleft}
\end{minipage}
\begin{minipage}[t]{0.4\textwidth}
\begin{flushright} \large
\emph{Supervisor:} \\
\href{http://www.jamessmith.com}{\supname} % Supervisor name - remove the \href bracket to remove the link  
\end{flushright}
\end{minipage}\\[1cm]
 
\vfill

\large \textit{A thesis submitted in fulfillment of the requirements\\ for the degree of \degreename}\\[0.3cm] % University requirement text
\textit{in the}\\[0.4cm]
\groupname\\\deptname\\[1cm] % Research group name and department name

\includegraphics[width=0.5\textwidth]{img/UniversiteitLeidenLogo}

\vfill

{\large \today}\\[4cm] % Date

%\includegraphics{Logo} % University/department logo - uncomment to place it
 
\vfill
\end{center}
\end{titlepage}

\cleardoublepage


==> tex/includes.tex <==
\usepackage[utf8]{inputenc}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{braket}
\usepackage{dirtytalk}
\usepackage[inline]{enumitem}
\usepackage{mathtools}
\usepackage{xspace}
\usepackage[colorlinks=true,linkcolor=blue, citecolor=blue]{hyperref}
\usepackage[nameinlink]{cleveref}

\usepackage{scalerel}
\usepackage[hang,flushmargin]{footmisc}
\usepackage{dsfont}
\usepackage[framemethod=tikz]{mdframed}
\usepackage{mfirstuc}
\usepackage{bm}
\usepackage{scalerel}
\usepackage{stmaryrd}

% \addtolength{\topmargin}{-2cm}
% \addtolength{\footskip}{2cm}
\setlength{\marginparwidth}{4cm} % for wider todonotes

% images/figure
\usepackage{caption}
\usepackage{subcaption}
\usepackage{float}
\usepackage{graphicx}
\usepackage[section]{placeins} % floats in sections
\usepackage{subcaption}
\usepackage{tikz}
    \usetikzlibrary{automata, shapes, positioning, arrows}
\usepackage{xparse}
\usepackage{array}
    \newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
    \newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
    \newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

% text format
\usepackage{multicol}
\usepackage{parskip}

% writing aids
\usepackage[textsize=tiny]{todonotes}

% commands
\usepackage{ifthen}


==> tex/traces/mod5d1_5-4.tex <==
\begin{figure}[ht]
	\centering
	\newcommand{\localwidth}{0.8\linewidth}
	\begin{subfigure}{\localwidth}
	$\begin{array}{ll}
		B_1 = & \nset{a_1} \\
		B_2 = & \nset{(a_1 \land \neg a_0), a_2} \\
		B_3 = & \nset{a_3, a_4, a_5, a_6} \\
		B_4 = & \nset{a_7} \\
		B_5 = & \nset{a_7 \land \neg a_6} \\
				 & \ldots
		% B_6 = & \nset{\nary[\land]{a_7, \neg a_2, \neg a_3, \neg a_4, \neg a_5, \neg a_6}} \\
		% B_7 = & \nset{\nary[\land]{a_7, \neg a_1, \neg a_2, \neg a_3, \neg a_4, \neg a_5, \neg a_6}} \\
	\end{array}$
	\caption{
		Delta-encoded list of blocked cubes after finding a trace for the
		\autoref{fig:graph:mod5d1} for 5 pebbles.
	}
	\end{subfigure}

	\medskip

	\begin{subfigure}{\localwidth}
	$\begin{array}{ll}
		B_1 = & \nset{a_1} \\
		B_2 = & \nset{a_2, a_3, a_4} \\
		B_3 = & \nset{
			(a_3 \land \neg a_1 \land \neg a_2), 
			(a_4 \land \neg a_1 \land \neg a_2), 
			a_5} \\
		B_4 = & \{\,
			(\nary[\land]{a_4, \neg a_0, \neg a_1, \neg a_2}),\
			(\nary[\land]{a_5, \neg a_0, \neg a_1, \neg a_2}), \\
				& \hfill (\nary[\land]{a_5, \neg a_4})\ a_6,\ a_7 \,\} \\
		B_5 = & \nset{a_7 \land \neg a_6} \\
				 & \ldots
		% B_6 = & 
		% \nset{\nary[\land]{a_7, \neg a_2, \neg a_3, \neg a_4, \neg a_5, \neg a_6}}\\
		% B_7 = & 
		% \nset{\nary[\land]{a_7, \neg a_1, \neg a_2, \neg a_3, \neg a_4, \neg a_5, \neg a_6}} \\
	\end{array}$
	\caption{
		Delta-encoded list of blocked cubes after finding a trace for the
		\autoref{fig:graph:mod5d1} for 5 pebbles.
	}
	\end{subfigure}
\end{figure}

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.4\linewidth]{img/dag/mod5d1}
	\caption{
		The directed acyclic graph representing the \texttt{mod5d1}
		\cite{rls-benchmarks}
	}
	\label{fig:graph:mod5d1}
\end{figure}

